Improving Adversarial Robustness for 3D Point Cloud Recognition at Test-Time through Purified Self-Training

Recognizing 3D point cloud plays a pivotal role in many real-world applications. However, deploying 3D point cloud deep learning model is vulnerable to adversarial attacks. Despite many efforts into developing robust model by adversarial training, they may become less effective against emerging attacks. This limitation motivates the development of adversarial purification which employs generative model to mitigate the impact of adversarial attacks. In this work, we highlight the remaining challenges from two perspectives. First, the purification based method requires retraining the classifier on purified samples which introduces additional computation overhead. Moreover, in a more realistic scenario, testing samples arrives in a streaming fashion and adversarial samples are not isolated from clean samples. These challenges motivates us to explore dynamically update model upon observing testing samples. We proposed a test-time purified self-training strategy to achieve this objective. Adaptive thresholding and feature distribution alignment are introduced to improve the robustness of self-training. Extensive results on different adversarial attacks suggest the proposed method is complementary to purification based method in handling continually changing adversarial attacks on the testing data stream.

==> sup_table/ablation.tex <==

\begin{tabular}{ccc|ccc|ccc}
\hline
 &  &  & \multicolumn{3}{c|}{White-box Attack} & \multicolumn{3}{c}{Adaptive Attack} \\ \hline
\multicolumn{1}{c|}{Self-Training} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Feature \\ Distribution \\ Alignment\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Point \\ Diffusion\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Clean \\ Acc.\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Avg. \\ Adv. Acc.\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Mixed \\ Acc.\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Clean \\ Acc.\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Avg. \\ Adv. Acc.\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Mixed \\ Acc.\end{tabular} \\ \hline
\multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - & \multicolumn{1}{c|}{41.4} & \multicolumn{1}{c|}{22.4} & 26.6 & \multicolumn{1}{c|}{47.9} & \multicolumn{1}{c|}{26.6} & 30.9 \\ \hline
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Fixed\\ Threshold\end{tabular}} & \multicolumn{1}{c|}{-} & - & \multicolumn{1}{c|}{40.6} & \multicolumn{1}{c|}{19.1} & 24.0 & \multicolumn{1}{c|}{38.0} & \multicolumn{1}{c|}{28.3} & 30.3 \\ \hline
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive\\ Threshold\end{tabular}} & \multicolumn{1}{c|}{-} & - & \multicolumn{1}{c|}{44.6} & \multicolumn{1}{c|}{21.1} & 26.4 & \multicolumn{1}{c|}{41.4} & \multicolumn{1}{c|}{33.5} & 35.1 \\ \hline
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive\\ Threshold\end{tabular}} & \multicolumn{1}{c|}{$\checkmark$} & - & \multicolumn{1}{c|}{51.2} & \multicolumn{1}{c|}{21.0} & 28.0 & \multicolumn{1}{c|}{46.7} & \multicolumn{1}{c|}{36.2} & 38.3 \\ \hline
\multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & PointDP & \multicolumn{1}{c|}{49.0} & \multicolumn{1}{c|}{26.7} & 32.3 & \multicolumn{1}{c|}{47.9} & \multicolumn{1}{c|}{28.5} & 32.4 \\ \hline
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Adaptive\\ Threshold\end{tabular}} & \multicolumn{1}{c|}{$\checkmark$} & PointDP & \multicolumn{1}{c|}{\textbf{52.1}} & \multicolumn{1}{c|}{\textbf{41.8}} & \textbf{44.3} & \multicolumn{1}{c|}{\textbf{50.2}} & \multicolumn{1}{c|}{\textbf{43.4}} & \textbf{44.8} \\ \hline
\end{tabular}


==> sup_table/adaptive_attack.tex <==

% \begin{tabular}{ccccccccccc|cccccccc}
% \hline
% \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{8}{c|}{Single Attack} & \multicolumn{8}{c}{Mixed Attack} \\ \cline{4-19} 
%  &  &  & \multicolumn{4}{c|}{\( l_\infty \)} & \multicolumn{4}{c|}{\( l_2 \)} & \multicolumn{4}{c|}{\( l_\infty \)} & \multicolumn{4}{c}{\( l_2 \)} \\ \cline{4-19} 
%  &  &  & BPDA-PGD & EOT-AutoAttack & PGD-Latent & \multicolumn{1}{c|}{AdvPC-Latent} & BPDA-PGD & EOT-AutoAttack & PGD-Latent & AdvPC-Latent & BPDA-PGD & EOT-AutoAttack & PGD-Latent & \multicolumn{1}{c|}{AdvPC-Latent} & BPDA-PGD & EOT-AutoAttack & PGD-Latent & AdvPC-Latent \\ \hline

\begin{tabular}{ccccccccccc|cccccccc}
\hline
\multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{8}{c|}{Single Attack} & \multicolumn{8}{c}{Mixed Attack} \\ \cline{4-19} 
 &  &  & \multicolumn{4}{c|}{\( l_\infty \)} & \multicolumn{4}{c|}{\( l_2 \)} & \multicolumn{4}{c|}{\( l_\infty \)} & \multicolumn{4}{c}{\( l_2 \)} \\ \cline{4-19} 
 &  &  & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BPDA-\\ PGD\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}EOT-\\ AutoAttack\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}PGD-\\ Latent\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}AdvPC-\\ Latent\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BPDA-\\ PGD\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}EOT-\\ AutoAttack\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}PGD-\\ Latent\end{tabular}} & \begin{tabular}[c]{@{}c@{}}AdvPC-\\ Latent\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BPDA-\\ PGD\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}EOT-\\ AutoAttack\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}PGD-\\ Latent\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}AdvPC-\\ Latent\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BPDA-\\ PGD\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}EOT-\\ AutoAttack\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}PGD-\\ Latent\end{tabular}} & \begin{tabular}[c]{@{}c@{}}AdvPC-\\ Latent\end{tabular} \\ \hline
\multirow{6}{*}{{\begin{sideways}PointNet\end{sideways}}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & 83.6 & 83.6 & 83.6 & \multicolumn{1}{c|}{83.6} & 83.6 & 83.6 & 83.6 & 83.6 & \multicolumn{4}{c|}{77.2} & \multicolumn{4}{c}{77.2} \\
 &  & Adv Acc & 69.7 & 62.5 & 69.7 & \multicolumn{1}{c|}{50.3} & 79.8 & 73.4 & 84.7 & 81.4 & 63.4 & 61.6 & 68.3 & \multicolumn{1}{c|}{63.4} & 75.6 & \textbf{72.4} & 84.9 & 94.1 \\
 &  & Mixed Acc & 76.7 & 73.1 & 76.7 & \multicolumn{1}{c|}{67.0} & 81.7 & 78.5 & 84.2 & 82.5 & \multicolumn{4}{c|}{66.8} & \multicolumn{4}{c}{80.8} \\ \cline{2-19} 
 & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \textbf{85.0} & \textbf{85.2} & \textbf{84.6} & \multicolumn{1}{c|}{\textbf{84.8}} & \textbf{85.3} & \textbf{84.6} & \textbf{84.7} & \textbf{85.1} & \multicolumn{4}{c|}{\textbf{78.1}} & \multicolumn{4}{c}{\textbf{78.2}} \\
 &  & Adv Acc & \textbf{73.6} & \textbf{68.9} & \textbf{76.5} & \multicolumn{1}{c|}{\textbf{54.6}} & \textbf{82.3} & \textbf{75.8} & \textbf{85.4} & \textbf{83.4} & \textbf{70.6} & \textbf{63.7} & \textbf{72.8} & \multicolumn{1}{c|}{\textbf{74.0}} & \textbf{79.3} & 71.0 & \textbf{87.2} & \textbf{94.5} \\
 &  & Mixed Acc & \textbf{79.3} & \textbf{77.1} & \textbf{80.6} & \multicolumn{1}{c|}{\textbf{69.7}} & \textbf{83.8} & \textbf{80.2} & \textbf{85.1} & \textbf{84.3} & \multicolumn{4}{c|}{\textbf{71.8}} & \multicolumn{4}{c}{\textbf{82.1}} \\ \hline \hline
\multirow{6}{*}{{\begin{sideways}DGCNN\end{sideways}}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & 74.1 & 74.1 & 74.1 & \multicolumn{1}{c|}{74.1} & 74.1 & 74.1 & 74.1 & 74.1 & \multicolumn{4}{c|}{66.3} & \multicolumn{4}{c}{66.3} \\
 &  & Adv Acc & 62.1 & 62.5 & 48.3 & \multicolumn{1}{c|}{43.2} & 62.9 & 72.1 & 82.0 & \textbf{73.9} & 60.0 & 62.1 & 39.9 & \multicolumn{1}{c|}{57.6} & 62.4 & 70.1 & 86.4 & 89.4 \\
 &  & Mixed Acc & 68.1 & 68.3 & 61.3 & \multicolumn{1}{c|}{58.7} & 68.6 & 73.1 & 78.1 & \textbf{74.0} & \multicolumn{4}{c|}{57.2} & \multicolumn{4}{c}{74.9} \\ \cline{2-19} 
 & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \textbf{80.8} & \textbf{80.9} & \textbf{80.4} & \multicolumn{1}{c|}{\textbf{79.1}} & \textbf{82.4} & \textbf{81.7} & \textbf{83.2} & \textbf{81.6} & \multicolumn{4}{c|}{\textbf{75.6}} & \multicolumn{4}{c}{\textbf{76.6}} \\
 &  & Adv Acc & \textbf{77.4} & \textbf{78.1} & \textbf{77.8} & \multicolumn{1}{c|}{\textbf{64.0}} & \textbf{77.1} & \textbf{80.9} & \textbf{88.4} & 65.6 & \textbf{74.1} & \textbf{70.8} & \textbf{80.1} & \multicolumn{1}{c|}{\textbf{86.6}} & \textbf{75.7} & \textbf{76.5} & \textbf{88.2} & \textbf{93.1} \\
 &  & Mixed Acc & \textbf{79.1} & \textbf{79.5} & \textbf{79.1} & \multicolumn{1}{c|}{\textbf{71.6}} & \textbf{79.8} & \textbf{81.3} & \textbf{85.8} & 73.6 & \multicolumn{4}{c|}{\textbf{77.4}} & \multicolumn{4}{c}{\textbf{82.0}} \\ \hline \hline
\multirow{6}{*}{{\begin{sideways}PointMLP\end{sideways}}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & 61.6 & 61.6 & 61.6 & \multicolumn{1}{c|}{61.6} & 61.6 & 61.6 & 61.6 & 61.6 & \multicolumn{4}{c|}{59.2} & \multicolumn{4}{c}{58.2} \\
 &  & Adv Acc & 37.3 & 38.9 & 15.8 & \multicolumn{1}{c|}{18.7} & 43.4 & 53.9 & 67.9 & 59.9 & 43.3 & 38.7 & 3.5 & \multicolumn{1}{c|}{12.3} & 52.5 & 53.3 & 57.6 & 70.5 \\
 &  & Mixed Acc & 49.5 & 50.3 & 38.7 & \multicolumn{1}{c|}{40.2} & 52.5 & 57.8 & 64.8 & 60.8 & \multicolumn{4}{c|}{31.4} & \multicolumn{4}{c}{58.6} \\ \cline{2-19} 
 & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \textbf{81.5} & \textbf{81.0} & \textbf{81.2} & \multicolumn{1}{c|}{\textbf{77.9}} & \textbf{80.4} & \textbf{82.0} & \textbf{81.4} & \textbf{80.3} & \multicolumn{4}{c|}{\textbf{78.4}} & \multicolumn{4}{c}{\textbf{78.4}} \\
 &  & Adv Acc & \textbf{80.7} & \textbf{78.7} & \textbf{80.5} & \multicolumn{1}{c|}{\textbf{61.9}} & \textbf{76.6} & \textbf{79.3} & \textbf{85.9} & \textbf{80.0} & \textbf{77.1} & \textbf{69.0} & \textbf{84.2} & \multicolumn{1}{c|}{\textbf{81.1}} & \textbf{76.7} & \textbf{76.1} & \textbf{86.4} & \textbf{90.3} \\
 &  & Mixed Acc & \textbf{81.1} & \textbf{79.8} & \textbf{80.9} & \multicolumn{1}{c|}{\textbf{70.0}} & \textbf{78.5} & \textbf{80.6} & \textbf{83.6} & \textbf{80.2} & \multicolumn{4}{c|}{\textbf{78.0}} & \multicolumn{4}{c}{\textbf{81.6}} \\ \hline
\end{tabular}


==> sup_table/bk.tex <==
\begin{table}[]
\centering
\vspace{-0.3cm}
\caption{Ablation study on ScanObjectNN dataset with PCT backbone.}
\setlength\tabcolsep{2pt} 
        \resizebox{0.99\linewidth}{!}{
\begin{tabular}{|c|c|c|ccc|ccc|}
\hline
 &  &  & \multicolumn{3}{c|}{White-box Attack} & \multicolumn{3}{c|}{Adaptive Attack} \\ \hline
Self-Training & \begin{tabular}[c]{@{}c@{}}Feature \\ Distribution \\ Alignment\end{tabular} & \begin{tabular}[c]{@{}c@{}}Point \\ Diffusion\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Clean \\ Acc.\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Avg. \\ Adv. Acc.\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Mixed \\ Acc.\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Clean \\ Acc.\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Avg. \\ Adv. Acc.\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Mixed \\ Acc.\end{tabular} \\ \hline
- & - & - & \multicolumn{1}{c|}{41.4} & \multicolumn{1}{c|}{22.4} & 26.6 & \multicolumn{1}{c|}{47.9} & \multicolumn{1}{c|}{26.6} & 30.9 \\ \hline
\begin{tabular}[c]{@{}c@{}}Fixed\\      Threshold\end{tabular} & - & - & \multicolumn{1}{c|}{40.6} & \multicolumn{1}{c|}{19.1} & 24.0 & \multicolumn{1}{c|}{38.0} & \multicolumn{1}{c|}{28.3} & 30.3 \\ \hline
\begin{tabular}[c]{@{}c@{}}Adaptive\\      Threshold\end{tabular} & - & - & \multicolumn{1}{c|}{44.6} & \multicolumn{1}{c|}{21.1} & 26.4 & \multicolumn{1}{c|}{41.4} & \multicolumn{1}{c|}{33.5} & 35.1 \\ \hline
\begin{tabular}[c]{@{}c@{}}Adaptive\\      Threshold\end{tabular} & $\checkmark$ & - & \multicolumn{1}{c|}{51.2} & \multicolumn{1}{c|}{21.0} & 28.0 & \multicolumn{1}{c|}{46.7} & \multicolumn{1}{c|}{36.2} & 38.3 \\ \hline
- & - & PointDP & \multicolumn{1}{c|}{49.0} & \multicolumn{1}{c|}{26.7} & 32.3 & \multicolumn{1}{c|}{47.9} & \multicolumn{1}{c|}{28.5} & 32.4 \\ \hline
\begin{tabular}[c]{@{}c@{}}Adaptive\\      Threshold\end{tabular} & $\checkmark$ & PointDP & \multicolumn{1}{c|}{\textbf{52.1}} & \multicolumn{1}{c|}{\textbf{41.8}} & \textbf{44.3} & \multicolumn{1}{c|}{\textbf{50.2}} & \multicolumn{1}{c|}{\textbf{43.4}} & \textbf{44.8} \\ \hline
\end{tabular}
}
\label{tab:ablation}%
\vspace{-0.5cm}
\end{table}




\begin{table}[]
\caption{Evaluation of adversarial performance with different backbone networks without adversarial training on ModelNet40 dataset.}
  \resizebox{0.99\linewidth}{!}{
\begin{tabular}{|cl|cccccccc|cccccccc|}
\hline
\multicolumn{2}{|l|}{\multirow{3}{*}{\textbf{}}}                       & \multicolumn{8}{c|}{Single Attack}                                                                                                                                                                                                                                               & \multicolumn{8}{c|}{Mixed Attack}                                                                                                                                                                                                                                             \\ \cline{3-18} 
\multicolumn{2}{|l|}{}                                                 & \multicolumn{4}{c|}{\( l_\infty \)}                                                                                                                        & \multicolumn{4}{c|}{\( l_2 \)}                                                                                                      & \multicolumn{4}{c|}{\( l_\infty \)}                                                                                                                      & \multicolumn{4}{c|}{\( l_2 \)}                                                                                                     \\ \cline{3-18} 
\multicolumn{2}{|l|}{}                                                 & \multicolumn{1}{c|}{C\&W}          & \multicolumn{1}{c|}{PGD}           & \multicolumn{1}{c|}{AdvPC}         & \multicolumn{1}{c|}{SI\_Adv}       & \multicolumn{1}{c|}{C\&W}          & \multicolumn{1}{c|}{PGD}           & \multicolumn{1}{c|}{AdvPC}         & KNN           & \multicolumn{1}{c|}{C\&W}         & \multicolumn{1}{c|}{PGD}          & \multicolumn{1}{c|}{AdvPC}         & \multicolumn{1}{c|}{SI\_Adv}       & \multicolumn{1}{c|}{C\&W}         & \multicolumn{1}{c|}{PGD}           & \multicolumn{1}{c|}{AdvPC}         & KNN           \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{PCT}}}        & Clean Acc & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \textbf{93.7} & \multicolumn{4}{c|}{\textbf{89.3}}                                                                                                              & \multicolumn{4}{c|}{\textbf{89.3}}                                                                                          \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Adv Acc   & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{27.6}} & \multicolumn{1}{c|}{\textbf{2.6}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \textbf{66.8} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{35.7}} & \multicolumn{1}{c|}{\textbf{2.2}} & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \textbf{70.3} \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Mixed Acc & \multicolumn{1}{c|}{\textbf{46.9}} & \multicolumn{1}{c|}{\textbf{46.9}} & \multicolumn{1}{c|}{\textbf{46.9}} & \multicolumn{1}{c|}{\textbf{60.7}} & \multicolumn{1}{c|}{\textbf{48.2}} & \multicolumn{1}{c|}{\textbf{46.9}} & \multicolumn{1}{c|}{\textbf{46.9}} & \textbf{80.2} & \multicolumn{4}{c|}{\textbf{25.1}}                                                                                                              & \multicolumn{4}{c|}{\textbf{32.4}}                                                                                          \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{PointNet\texttt{++}}}} & Clean Acc & \multicolumn{1}{c|}{\textbf{92.9}} & \multicolumn{1}{c|}{\textbf{92.9}} & \multicolumn{1}{c|}{\textbf{92.9}} & \multicolumn{1}{c|}{\textbf{92.9}} & \multicolumn{1}{c|}{\textbf{92.9}} & \multicolumn{1}{c|}{\textbf{92.9}} & \multicolumn{1}{c|}{\textbf{92.9}} & \textbf{92.9} & \multicolumn{4}{c|}{\textbf{89.3}}                                                                                                              & \multicolumn{4}{c|}{\textbf{89.3}}                                                                                          \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Adv Acc   & \multicolumn{1}{c|}{\textbf{1.2}}  & \multicolumn{1}{c|}{\textbf{3.5}}  & \multicolumn{1}{c|}{\textbf{3.8}}  & \multicolumn{1}{c|}{\textbf{8.0}}  & \multicolumn{1}{c|}{\textbf{1.7}}  & \multicolumn{1}{c|}{\textbf{14.1}} & \multicolumn{1}{c|}{\textbf{3.8}}  & \textbf{42.8} & \multicolumn{1}{c|}{\textbf{0.8}} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{1}{c|}{\textbf{12.5}} & \multicolumn{1}{c|}{\textbf{20.4}} & \multicolumn{1}{c|}{\textbf{1.4}} & \multicolumn{1}{c|}{\textbf{2.2}}  & \multicolumn{1}{c|}{\textbf{12.5}} & \textbf{40.7} \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Mixed Acc & \multicolumn{1}{c|}{\textbf{47.1}} & \multicolumn{1}{c|}{\textbf{48.3}} & \multicolumn{1}{c|}{\textbf{48.4}} & \multicolumn{1}{c|}{\textbf{50.5}} & \multicolumn{1}{c|}{\textbf{47.3}} & \multicolumn{1}{c|}{\textbf{53.5}} & \multicolumn{1}{c|}{\textbf{48.4}} & \textbf{67.9} & \multicolumn{4}{c|}{\textbf{24.5}}                                                                                                              & \multicolumn{4}{c|}{\textbf{29.3}}                                                                                          \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{CurveNet}}}   & Clean Acc & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \textbf{93.7} & \multicolumn{4}{c|}{\textbf{90.7}}                                                                                                              & \multicolumn{4}{c|}{\textbf{90.7}}                                                                                          \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Adv Acc   & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{32.4}} & \multicolumn{1}{c|}{\textbf{3.9}}  & \multicolumn{1}{c|}{\textbf{3.1}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \textbf{70.7} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{25.7}} & \multicolumn{1}{c|}{\textbf{3.2}} & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \textbf{72.0} \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Mixed Acc & \multicolumn{1}{c|}{\textbf{46.9}} & \multicolumn{1}{c|}{\textbf{46.9}} & \multicolumn{1}{c|}{\textbf{46.9}} & \multicolumn{1}{c|}{\textbf{63.1}} & \multicolumn{1}{c|}{\textbf{48.9}} & \multicolumn{1}{c|}{\textbf{48.5}} & \multicolumn{1}{c|}{\textbf{46.9}} & \textbf{82.2} & \multicolumn{4}{c|}{\textbf{23.2}}                                                                                                              & \multicolumn{4}{c|}{\textbf{33.2}}                                                                                          \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{PointNet}}}   & Clean Acc & \multicolumn{1}{c|}{\textbf{91.5}} & \multicolumn{1}{c|}{\textbf{91.5}} & \multicolumn{1}{c|}{\textbf{91.5}} & \multicolumn{1}{c|}{\textbf{91.5}} & \multicolumn{1}{c|}{\textbf{91.5}} & \multicolumn{1}{c|}{\textbf{91.5}} & \multicolumn{1}{c|}{\textbf{91.5}} & \textbf{91.5} & \multicolumn{4}{c|}{\textbf{85.6}}                                                                                                              & \multicolumn{4}{c|}{\textbf{85.6}}                                                                                          \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Adv Acc   & \multicolumn{1}{c|}{\textbf{2.3}}  & \multicolumn{1}{c|}{\textbf{1.7}}  & \multicolumn{1}{c|}{\textbf{2.2}}  & \multicolumn{1}{c|}{\textbf{47.9}} & \multicolumn{1}{c|}{\textbf{2.6}}  & \multicolumn{1}{c|}{\textbf{28.6}} & \multicolumn{1}{c|}{\textbf{2.2}}  & \textbf{54.4} & \multicolumn{1}{c|}{\textbf{1.2}} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{1}{c|}{\textbf{10.7}} & \multicolumn{1}{c|}{\textbf{62.2}} & \multicolumn{1}{c|}{\textbf{1.8}} & \multicolumn{1}{c|}{\textbf{31.0}} & \multicolumn{1}{c|}{\textbf{10.7}} & \textbf{61.4} \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Mixed Acc & \multicolumn{1}{c|}{\textbf{46.9}} & \multicolumn{1}{c|}{\textbf{46.6}} & \multicolumn{1}{c|}{\textbf{46.9}} & \multicolumn{1}{c|}{\textbf{69.7}} & \multicolumn{1}{c|}{\textbf{47.1}} & \multicolumn{1}{c|}{\textbf{60.1}} & \multicolumn{1}{c|}{\textbf{46.9}} & \textbf{73.0} & \multicolumn{4}{c|}{\textbf{31.9}}                                                                                                              & \multicolumn{4}{c|}{\textbf{38.2}}                                                                                          \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{DGCNN}}}      & Clean Acc & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \multicolumn{1}{c|}{\textbf{93.7}} & \textbf{93.7} & \multicolumn{4}{c|}{\textbf{88.1}}                                                                                                              & \multicolumn{4}{c|}{\textbf{88.1}}                                                                                          \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Adv Acc   & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{2.5}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.4}}  & \textbf{52.7} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{1}{c|}{\textbf{0.2}}  & \multicolumn{1}{c|}{\textbf{0.4}}  & \multicolumn{1}{c|}{\textbf{2.2}} & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{1.2}}  & \textbf{55.5} \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Mixed Acc & \multicolumn{1}{c|}{\textbf{46.9}} & \multicolumn{1}{c|}{\textbf{46.9}} & \multicolumn{1}{c|}{\textbf{46.9}} & \multicolumn{1}{c|}{\textbf{46.9}} & \multicolumn{1}{c|}{\textbf{48.1}} & \multicolumn{1}{c|}{\textbf{46.9}} & \multicolumn{1}{c|}{\textbf{47.1}} & \textbf{73.2} & \multicolumn{4}{c|}{\textbf{17.7}}                                                                                                              & \multicolumn{4}{c|}{\textbf{29.5}}                                                                                          \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{PointMLP}}}   & Clean Acc & \multicolumn{1}{c|}{\textbf{94.9}} & \multicolumn{1}{c|}{\textbf{94.9}} & \multicolumn{1}{c|}{\textbf{94.9}} & \multicolumn{1}{c|}{\textbf{94.9}} & \multicolumn{1}{c|}{\textbf{94.9}} & \multicolumn{1}{c|}{\textbf{94.9}} & \multicolumn{1}{c|}{\textbf{94.9}} & \textbf{94.9} & \multicolumn{4}{c|}{\textbf{91.1}}                                                                                                              & \multicolumn{4}{c|}{\textbf{91.1}}                                                                                          \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Adv Acc   & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{41.8}} & \multicolumn{1}{c|}{\textbf{2.0}}  & \multicolumn{1}{c|}{\textbf{0.2}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \textbf{35.6} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{48.6}} & \multicolumn{1}{c|}{\textbf{1.2}} & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \textbf{43.6} \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Mixed Acc & \multicolumn{1}{c|}{\textbf{47.5}} & \multicolumn{1}{c|}{\textbf{47.5}} & \multicolumn{1}{c|}{\textbf{47.5}} & \multicolumn{1}{c|}{\textbf{68.4}} & \multicolumn{1}{c|}{\textbf{48.5}} & \multicolumn{1}{c|}{\textbf{47.6}} & \multicolumn{1}{c|}{\textbf{47.5}} & \textbf{65.3} & \multicolumn{4}{c|}{\textbf{27.9}}                                                                                                              & \multicolumn{4}{c|}{\textbf{27.2}}                                                                                          \\ \hline
\end{tabular}
}
\label{tab:base_modelnet40}%\
\end{table}



\begin{table}[]
\caption{Evaluation of adversarial performance with different backbone networks without adversarial training on ScanObjectNN dataset.}
  \resizebox{0.99\linewidth}{!}{
\begin{tabular}{|cl|ccclcccc|ccclcccc|}
\hline
\multicolumn{2}{|l|}{\multirow{3}{*}{\textbf{}}}                       & \multicolumn{8}{c|}{Single Attack}                                                                                                                                                                                                          & \multicolumn{8}{c|}{Mixed Attack}                                                                                                                                                                                                     \\ \cline{3-18} 
\multicolumn{2}{|l|}{}                                                 & \multicolumn{4}{c|}{\( l_\infty \)}                                                                                   & \multicolumn{4}{c|}{\( l_2 \)}                                                                                                      & \multicolumn{4}{c|}{\( l_\infty \)}                                                                                & \multicolumn{4}{c|}{\( l_2 \)}                                                                                                   \\ \cline{3-18} 
\multicolumn{2}{|l|}{}                                                 & \multicolumn{1}{c|}{C\&W}          & \multicolumn{1}{c|}{PGD}           & \multicolumn{2}{c|}{AdvPC}         & \multicolumn{1}{c|}{C\&W}          & \multicolumn{1}{c|}{PGD}           & \multicolumn{1}{c|}{AdvPC}         & KNN           & \multicolumn{1}{c|}{C\&W}         & \multicolumn{1}{c|}{PGD}          & \multicolumn{2}{c|}{AdvPC}        & \multicolumn{1}{c|}{C\&W}         & \multicolumn{1}{c|}{PGD}          & \multicolumn{1}{c|}{AdvPC}        & KNN           \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{PCT}}}        & Clean Acc & \multicolumn{1}{c|}{\textbf{78.4}} & \multicolumn{1}{c|}{\textbf{78.4}} & \multicolumn{2}{c|}{\textbf{78.4}} & \multicolumn{1}{c|}{\textbf{78.4}} & \multicolumn{1}{c|}{\textbf{78.4}} & \multicolumn{1}{c|}{\textbf{78.4}} & \textbf{78.4} & \multicolumn{4}{c|}{\textbf{75.5}}                                                                        & \multicolumn{4}{c|}{\textbf{82.4}}                                                                                        \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Adv Acc   & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{2}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{4.8}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \textbf{25.3} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{2}{c|}{\textbf{0.0}} & \multicolumn{1}{c|}{\textbf{4.3}} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{1}{c|}{\textbf{0.0}} & \textbf{23.1} \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Mixed Acc & \multicolumn{1}{c|}{\textbf{39.2}} & \multicolumn{1}{c|}{\textbf{39.2}} & \multicolumn{2}{c|}{\textbf{39.2}} & \multicolumn{1}{c|}{\textbf{41.6}} & \multicolumn{1}{c|}{\textbf{39.2}} & \multicolumn{1}{c|}{\textbf{39.2}} & \textbf{51.9} & \multicolumn{4}{c|}{\textbf{18.8}}                                                                        & \multicolumn{4}{c|}{\textbf{22.0}}                                                                                        \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{PointNet\texttt{++}}}} & Clean Acc & \multicolumn{1}{c|}{\textbf{80.1}} & \multicolumn{1}{c|}{\textbf{80.1}} & \multicolumn{2}{c|}{\textbf{80.1}} & \multicolumn{1}{c|}{\textbf{80.1}} & \multicolumn{1}{c|}{\textbf{80.1}} & \multicolumn{1}{c|}{\textbf{80.1}} & \textbf{80.1} & \multicolumn{4}{c|}{\textbf{80.1}}                                                                        & \multicolumn{4}{c|}{\textbf{81.7}}                                                                                        \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Adv Acc   & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{2}{c|}{\textbf{0.1}}  & \multicolumn{1}{c|}{\textbf{2.4}}  & \multicolumn{1}{c|}{\textbf{4.5}}  & \multicolumn{1}{c|}{\textbf{1.3}}  & \textbf{16.4} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{2}{c|}{\textbf{0.1}} & \multicolumn{1}{c|}{\textbf{1.3}} & \multicolumn{1}{c|}{\textbf{5.2}} & \multicolumn{1}{c|}{\textbf{0.8}} & \textbf{11.9} \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Mixed Acc & \multicolumn{1}{c|}{\textbf{40.1}} & \multicolumn{1}{c|}{\textbf{40.1}} & \multicolumn{2}{c|}{\textbf{40.1}} & \multicolumn{1}{c|}{\textbf{41.3}} & \multicolumn{1}{c|}{\textbf{42.3}} & \multicolumn{1}{c|}{\textbf{40.7}} & \textbf{48.3} & \multicolumn{4}{c|}{\textbf{20.0}}                                                                        & \multicolumn{4}{c|}{\textbf{20.1}}                                                                                        \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{CurveNet}}}   & Clean Acc & \multicolumn{1}{c|}{\textbf{78.7}} & \multicolumn{1}{c|}{\textbf{78.7}} & \multicolumn{2}{c|}{\textbf{78.7}} & \multicolumn{1}{c|}{\textbf{78.7}} & \multicolumn{1}{c|}{\textbf{78.7}} & \multicolumn{1}{c|}{\textbf{78.7}} & \textbf{78.7} & \multicolumn{4}{c|}{\textbf{77.2}}                                                                        & \multicolumn{4}{c|}{\textbf{81.7}}                                                                                        \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Adv Acc   & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{1}{c|}{\textbf{0.0}}  & \multicolumn{2}{c|}{\textbf{0.2}}  & \multicolumn{1}{c|}{\textbf{3.9}}  & \multicolumn{1}{c|}{\textbf{1.4}}  & \multicolumn{1}{c|}{\textbf{0.6}}  & \textbf{34.7} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{1}{c|}{\textbf{0.0}} & \multicolumn{2}{c|}{\textbf{0.2}} & \multicolumn{1}{c|}{\textbf{2.7}} & \multicolumn{1}{c|}{\textbf{1.2}} & \multicolumn{1}{c|}{\textbf{1.8}} & \textbf{29.8} \\ \cline{2-18} 
\multicolumn{1}{|c|}{}                                     & Mixed Acc & \multicolumn{1}{c|}{\textbf{39.4}} & \multicolumn{1}{c|}{\textbf{39.4}} & \multicolumn{2}{c|}{\textbf{39.5}} & \multicolumn{1}{c|}{\textbf{41.3}} & \multicolumn{1}{c|}{\textbf{40.1}} & \multicolumn{1}{c|}{\textbf{39.6}} & \textbf{56.8} & \multicolumn{4}{c|}{\textbf{19.3}}                                                                        & \multicolumn{4}{c|}{\textbf{23.4}}                                                                                        \\ \hline
\end{tabular}
}
\label{tab:base_scanobjnn}
\end{table}

\begin{table}[]
\caption{Evaluation of robustness against adaptive attacks on ModelNet40 dataset on additional backbones. Both Single Attack and Mixed Attack are reported on five types of adaptive adversarial
attacks. }
  \resizebox{0.99\linewidth}{!}{
\begin{tabular}{|ccl|cccccccc|cccccccc|}
\hline
\multicolumn{3}{|l|}{}                                                                                                                                     & \multicolumn{8}{c|}{Single Attack}                                                                                                                                                                                                                                                                                                                                                                                                                                               & \multicolumn{8}{c|}{Mixed Attack}                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \cline{4-19} 
\multicolumn{3}{|l|}{}                                                                                                                                     & \multicolumn{4}{c|}{\( l_\infty \)}                                                                                                                                                                                                                        & \multicolumn{4}{c|}{\( l_2 \)}                                                                                                                                                                                                      & \multicolumn{4}{c|}{\( l_\infty \)}                                                                                                                                                                                                                        & \multicolumn{4}{c|}{\( l_2 \)}                                                                                                                                                                                                      \\ \cline{4-19} 
\multicolumn{3}{|l|}{\multirow{-3}{*}{}}                                                                                                                   & \multicolumn{1}{c|}{BPDA- PGD}                             & \multicolumn{1}{c|}{EOT-AutoAttack}                        & \multicolumn{1}{c|}{PGD-Latent}                            & \multicolumn{1}{c|}{AdvPC-Latent}                          & \multicolumn{1}{c|}{BPDA-PGD}                              & \multicolumn{1}{c|}{EOT-AutoAttack}                        & \multicolumn{1}{c|}{PGD-Latent}                            & AdvPC-Latent                          & \multicolumn{1}{c|}{BPDA- PGD}                             & \multicolumn{1}{c|}{EOT-AutoAttack}                        & \multicolumn{1}{c|}{PGD-Latent}                            & \multicolumn{1}{c|}{AdvPC-Latent}                          & \multicolumn{1}{c|}{BPDA-PGD}                              & \multicolumn{1}{c|}{EOT-AutoAttack}                        & \multicolumn{1}{c|}{PGD-Latent}                            & AdvPC-Latent                          \\ \hline
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                                      & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}83.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}83.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}83.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}83.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}83.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}83.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}83.6}          & \cellcolor[HTML]{FBDAD7}83.6          & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}77.2}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}77.2}                                                                                                                                                                            \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                                      & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}69.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}62.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}69.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}50.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}79.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}73.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}84.7}          & \cellcolor[HTML]{FEF2CD}81.4          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}63.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}61.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}68.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}63.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}75.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{72.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}84.9}          & \cellcolor[HTML]{FEF2CD}94.1          \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{\multirow{-3}{*}{Pt. DP}}              & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}76.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}73.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}76.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}67.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}81.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}78.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}84.2}          & \cellcolor[HTML]{D9E7FD}82.5          & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}66.8}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}80.8}                                                                                                                                                                            \\ \cline{2-19} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                                      & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{85.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{85.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{85.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.7}} & \cellcolor[HTML]{FBDAD7}\textbf{85.1} & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{78.1}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{78.2}}                                                                                                                                                                   \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                                      & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{73.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{68.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{76.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{54.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{82.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{75.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{85.4}} & \cellcolor[HTML]{FEF2CD}\textbf{83.4} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{70.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{63.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{72.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{74.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{79.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}71.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{87.2}} & \cellcolor[HTML]{FEF2CD}\textbf{94.5} \\ \cline{3-19} 
\multicolumn{1}{|c|}{\multirow{-6}{*}{\textbf{PointNet}}} & \multicolumn{1}{c|}{\multirow{-3}{*}{Pt. DP+ S.T. (Ours)}} & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{77.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{80.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{69.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{83.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{80.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{85.1}} & \cellcolor[HTML]{D9E7FD}\textbf{84.3} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{71.8}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{82.1}}                                                                                                                                                                   \\ \hline
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                                      & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}74.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}74.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}74.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}74.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}74.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}74.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}74.1}          & \cellcolor[HTML]{FBDAD7}74.1          & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}66.3}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}66.3}                                                                                                                                                                            \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                                      & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}62.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}62.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}48.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}43.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}62.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}72.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}82.0}          & \cellcolor[HTML]{FEF2CD}\textbf{73.9} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}60.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}62.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}39.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}57.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}62.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}70.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}86.4}          & \cellcolor[HTML]{FEF2CD}89.4          \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{\multirow{-3}{*}{Pt. DP}}              & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}68.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}68.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}61.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}58.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}68.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}73.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}78.1}          & \cellcolor[HTML]{D9E7FD}\textbf{74.0} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}57.2}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}74.9}                                                                                                                                                                            \\ \cline{2-19} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                                      & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{80.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{80.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{80.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{79.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{82.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{81.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.2}} & \cellcolor[HTML]{FBDAD7}\textbf{81.6} & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{75.6}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{76.6}}                                                                                                                                                                   \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                                      & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{77.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{78.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{77.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{64.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{77.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{80.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{88.4}} & \cellcolor[HTML]{FEF2CD}65.6          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{74.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{70.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{80.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{86.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{75.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{76.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{88.2}} & \cellcolor[HTML]{FEF2CD}\textbf{93.1} \\ \cline{3-19} 
\multicolumn{1}{|c|}{\multirow{-6}{*}{\textbf{DGCNN}}}    & \multicolumn{1}{c|}{\multirow{-3}{*}{Pt. DP+ S.T. (Ours)}} & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{71.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{85.8}} & \cellcolor[HTML]{D9E7FD}73.6          & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{77.4}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{82.0}}                                                                                                                                                                   \\ \hline
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                                      & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}61.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}61.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}61.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}61.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}61.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}61.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}61.6}          & \cellcolor[HTML]{FBDAD7}61.6          & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}59.2}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}58.2}                                                                                                                                                                            \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                                      & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}37.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}38.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}15.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}18.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}43.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}53.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}67.9}          & \cellcolor[HTML]{FEF2CD}59.9          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}43.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}38.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}3.5}           & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}12.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}52.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}53.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}57.6}          & \cellcolor[HTML]{FEF2CD}70.5          \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{\multirow{-3}{*}{Pt. DP}}              & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}49.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}50.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}38.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}40.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}52.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}57.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}64.8}          & \cellcolor[HTML]{D9E7FD}60.8          & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}31.4}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}58.6}                                                                                                                                                                            \\ \cline{2-19} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                                      & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{81.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{81.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{81.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{77.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{80.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{82.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{81.4}} & \cellcolor[HTML]{FBDAD7}\textbf{80.3} & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{78.4}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{78.4}}                                                                                                                                                                   \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                                      & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{80.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{78.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{80.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{61.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{76.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{79.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{85.9}} & \cellcolor[HTML]{FEF2CD}\textbf{80.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{77.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{69.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{84.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{81.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{76.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{76.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{86.4}} & \cellcolor[HTML]{FEF2CD}\textbf{90.3} \\ \cline{3-19} 
\multicolumn{1}{|c|}{\multirow{-6}{*}{\textbf{PointMLP}}} & \multicolumn{1}{c|}{\multirow{-3}{*}{Pt. DP+ S.T. (Ours)}} & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{80.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{70.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{78.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{80.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{83.6}} & \cellcolor[HTML]{D9E7FD}\textbf{80.2} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{78.0}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.6}}                                                                                                                                                                   \\ \hline
\end{tabular}
}
\label{tab:add_backbone_adaptive}
\end{table}


==> sup_table/md40_mix_attack.tex <==

\begin{tabular}{cllcccc|cccc}
\hline
\multicolumn{1}{l}{} &  &  & \multicolumn{4}{c|}{\( l_\infty \)} & \multicolumn{4}{c}{\( l_2 \)} \\ \cline{4-11} 
\multicolumn{1}{l}{} &  &  & C\&W & PGD & AdvPC & SI\_Adv & C\&W & PGD & AdvPC & KNN \\ \hline
\multirow{12}{*}{{\begin{sideways}PointNet\end{sideways}}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & \multicolumn{4}{c|}{77.2} & \multicolumn{4}{c}{77.2} \\
 &  & Adv Acc & 72.6 & 68.7 & 71.6 & 77.6 & 74.4 & 65.3 & 71.6 & \textbf{80.5} \\
 &  & Mixed Acc & \multicolumn{4}{c|}{73.5} & \multicolumn{4}{c}{73.8} \\ \cline{2-11} 
 & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \multicolumn{4}{c|}{\textbf{78}} & \multicolumn{4}{c}{\textbf{78.2}} \\
 &  & Adv Acc & \textbf{75.5} & \textbf{78.3} & \textbf{83.2} & \textbf{72.6} & \textbf{79.3} & \textbf{71.2} & \textbf{81.1} & 78.1 \\
 &  & Mixed Acc & \multicolumn{4}{c|}{\textbf{77.5}} & \multicolumn{4}{c}{\textbf{77.6}} \\ \cline{2-11} 
 & \multirow{3}{*}{IF-Def~\cite{wu2021ifdefense}} & Clean Acc & \multicolumn{4}{c|}{82.8} & \multicolumn{4}{c}{83} \\
 &  & Adv Acc & 79.5 & 72.4 & 67.3 & \textbf{82.3} & 81.5 & 81.5 & 66.5 & \textbf{80.7} \\
 &  & Mixed Acc & \multicolumn{4}{c|}{76.9} & \multicolumn{4}{c}{78.6} \\ \cline{2-11} 
 & \multirow{3}{*}{IF-Def+PST(Ours)} & Clean Acc & \multicolumn{4}{c|}{\textbf{83.5}} & \multicolumn{4}{c}{\textbf{83.3}} \\
 &  & Adv Acc & \textbf{81.3} & \textbf{75.5} & \textbf{77.1} & 81.1 & \textbf{84.6} & \textbf{85.8} & \textbf{75.1} & 79.7 \\
 &  & Mixed Acc & \multicolumn{4}{c|}{\textbf{79.7}} & \multicolumn{4}{c}{\textbf{81.7}} \\ \hline \hline
\multirow{12}{*}{{\begin{sideways}DGCNN\end{sideways}}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & \multicolumn{4}{c|}{66.3} & \multicolumn{4}{c}{66.3} \\
 &  & Adv Acc & 65.1 & 61.8 & 79.5 & 66.5 & 60.2 & 44.2 & 78.1 & 69.1 \\
 &  & Mixed Acc & \multicolumn{4}{c|}{67.8} & \multicolumn{4}{c}{63.6} \\ \cline{2-11} 
 & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \multicolumn{4}{c|}{\textbf{76.4}} & \multicolumn{4}{c}{\textbf{74.8}} \\
 &  & Adv Acc & \textbf{79.7} & \textbf{80.3} & \textbf{91.5} & \textbf{68} & \textbf{78.9} & \textbf{73.8} & \textbf{91.9} & \textbf{71.2} \\
 &  & Mixed Acc & \multicolumn{4}{c|}{\textbf{79.2}} & \multicolumn{4}{c}{\textbf{78.1}} \\ \cline{2-11} 
 & \multirow{3}{*}{IF-Def~\cite{wu2021ifdefense}} & Clean Acc & \multicolumn{4}{c|}{76.6} & \multicolumn{4}{c}{75.8} \\
 &  & Adv Acc & 75.2 & 65.9 & 77.4 & \textbf{79.1} & 73 & 76.2 & 77.6 & \textbf{81.1} \\
 &  & Mixed Acc & \multicolumn{4}{c|}{74.8} & \multicolumn{4}{c}{76.7} \\ \cline{2-11} 
 & \multirow{3}{*}{IF-Def+PST(Ours)} & Clean Acc & \multicolumn{4}{c|}{\textbf{80.7}} & \multicolumn{4}{c}{\textbf{81.9}} \\
 &  & Adv Acc & \textbf{81.3} & \textbf{81.1} & \textbf{88.6} & 73.2 & \textbf{76.3} & \textbf{81.5} & \textbf{88} & 75.9 \\
 &  & Mixed Acc & \multicolumn{4}{c|}{\textbf{81}} & \multicolumn{4}{c}{\textbf{80.7}} \\ \hline \hline
\multirow{12}{*}{{\begin{sideways}PointMLP\end{sideways}}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & \multicolumn{4}{c|}{59.2} & \multicolumn{4}{c}{59.2} \\
 &  & Adv Acc & 57.4 & 28.4 & 37.1 & 53.5 & 49.1 & 24.3 & 37.1 & \textbf{57.6} \\
 &  & Mixed Acc & \multicolumn{4}{c|}{47.1} & \multicolumn{4}{c}{45.5} \\ \cline{2-11} 
 & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \multicolumn{4}{c|}{\textbf{74.6}} & \multicolumn{4}{c}{\textbf{76}} \\
 &  & Adv Acc & \textbf{76.5} & \textbf{80.1} & \textbf{88.4} & \textbf{74.1} & \textbf{75.3} & \textbf{80.7} & \textbf{86.6} & \textbf{74.7} \\
 &  & Mixed Acc & \multicolumn{4}{c|}{\textbf{78.7}} & \multicolumn{4}{c}{\textbf{78.7}} \\ \cline{2-11} 
 & \multirow{3}{*}{IF-Def~\cite{wu2021ifdefense}} & Clean Acc & \multicolumn{4}{c|}{\textbf{82.2}} & \multicolumn{4}{c}{81.4} \\
 &  & Adv Acc & 75 & 57.2 & 75.8 & \textbf{78.5} & 73.6 & 71.6 & 78.5 & \textbf{77.2} \\
 &  & Mixed Acc & \multicolumn{4}{c|}{73.7} & \multicolumn{4}{c}{76.5} \\ \cline{2-11} 
 & \multirow{3}{*}{IF-Def+PST(Ours)} & Clean Acc & \multicolumn{4}{c|}{\textbf{81.5}} & \multicolumn{4}{c}{\textbf{82.5}} \\
 &  & Adv Acc & \textbf{76.3} & \textbf{80.7} & \textbf{85.6} & \textbf{78.6} & \textbf{77.1} & \textbf{82.6} & \textbf{88.3} & \textbf{76.3} \\
 &  & Mixed Acc & \multicolumn{4}{c|}{\textbf{80.5}} & \multicolumn{4}{c}{\textbf{81.3}} \\ \hline
\end{tabular}


==> sup_table/md40_single_attack.tex <==

\begin{tabular}{cllcccc|cccc}
\hline
 &  &  & \multicolumn{4}{c|}{\( l_\infty \)} & \multicolumn{4}{c}{\( l_2 \)} \\ \cline{4-11} 
 &  &  & C\&W & PGD & AdvPC & SI\_Adv & C\&W & PGD & AdvPC & KNN \\ \hline
\multirow{12}{*}{{\begin{sideways}PointNet\end{sideways}}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & 83.6 & 83.6 & 83.6 & 83.6 & 83.6 & 83.6 & 83.6 & 83.6 \\
 &  & Adv Acc & 77.0 & 64.5 & 57.3 & 76.8 & 77.2 & 62.7 & 57.1 & 79.5 \\
 &  & Mixed Acc & 80.3 & 74.1 & 70.5 & 80.2 & 80.4 & 73.2 & 70.3 & 81.6 \\ \cline{2-11} 
 & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \textbf{85.4} & \textbf{85.0} & \textbf{84.7} & \textbf{84.2} & \textbf{85.2} & \textbf{85.3} & \textbf{84.0} & \textbf{84.0} \\
 &  & Adv Acc & \textbf{79.6} & \textbf{71.6} & \textbf{64.6} & \textbf{79.0} & \textbf{79.6} & \textbf{67.7} & \textbf{63.8} & \textbf{83.2} \\
 &  & Mixed Acc & \textbf{82.5} & \textbf{78.3} & \textbf{74.7} & \textbf{81.6} & \textbf{82.4} & \textbf{76.5} & \textbf{74.0} & \textbf{83.7} \\ \cline{2-11} 
 & \multirow{3}{*}{IF-Def~\cite{wu2021ifdefense}} & Clean Acc & 82.0 & 81.5 & 83.0 & 81.6 & 82.3 & 81.7 & 82.2 & 82.2 \\
 &  & Adv Acc & 83.0 & 68.7 & 62.5 & 84.9 & 84.9 & 79.2 & 62.0 & 83.8 \\
 &  & Mixed Acc & 82.5 & 75.1 & 72.8 & 83.3 & 83.6 & 80.4 & 72.1 & 83.0 \\ \cline{2-11} 
 & \multirow{3}{*}{IF-Def+PST(Ours)} & Clean Acc & \textbf{83.0} & \textbf{83.3} & \textbf{83.7} & \textbf{82.9} & \textbf{83.0} & \textbf{82.9} & \textbf{82.7} & \textbf{83.0} \\
 &  & Adv Acc & \textbf{83.9} & \textbf{73.0} & \textbf{67.9} & \textbf{86.4} & \textbf{85.7} & \textbf{81.6} & \textbf{66.0} & \textbf{84.9} \\
 &  & Mixed Acc & \textbf{83.4} & \textbf{78.2} & \textbf{75.9} & \textbf{84.7} & \textbf{84.4} & \textbf{82.3} & \textbf{74.4} & \textbf{84.0} \\ \hline \hline
\multirow{12}{*}{{\begin{sideways}DGCNN\end{sideways}}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & 74.2 & 74.2 & 74.2 & 74.2 & 74.2 & 74.2 & 74.2 & 74.2 \\
 &  & Adv Acc & 68.8 & 62.3 & 59.9 & 70.7 & 61.2 & 54.7 & 58.6 & 74.7 \\
 &  & Mixed Acc & 71.5 & 68.2 & 67.1 & 72.5 & 67.7 & 64.5 & 66.4 & 74.4 \\ \cline{2-11} 
 & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \textbf{80.9} & \textbf{80.2} & \textbf{81.6} & \textbf{80.8} & \textbf{81.2} & \textbf{80.8} & \textbf{80.4} & \textbf{81.0} \\
 &  & Adv Acc & \textbf{76.8} & \textbf{76.0} & \textbf{74.7} & \textbf{80.0} & \textbf{77.1} & \textbf{72.6} & \textbf{74.3} & \textbf{80.8} \\
 &  & Mixed Acc & \textbf{78.9} & \textbf{78.1} & \textbf{78.2} & \textbf{80.4} & \textbf{79.2} & \textbf{76.7} & \textbf{77.4} & \textbf{81.0} \\ \cline{2-11} 
 & \multirow{3}{*}{IF-Def~\cite{wu2021ifdefense}} & Clean Acc & 75.8 & 74.1 & 75.0 & 74.5 & 75.4 & 74.3 & 76.3 & 74.3 \\
 &  & Adv Acc & 80.0 & 62.7 & 61.2 & 81.3 & 75.5 & 71.7 & 62.5 & 82.2 \\
 &  & Mixed Acc & 77.9 & 68.4 & 68.1 & 77.9 & 75.5 & 73.0 & 69.4 & 78.2 \\ \cline{2-11} 
 & \multirow{3}{*}{IF-Def+PST(Ours)} & Clean Acc & \textbf{78.3} & \textbf{78.0} & \textbf{78.3} & \textbf{81.2} & \textbf{78.3} & \textbf{78.6} & \textbf{78.2} & \textbf{77.8} \\
 &  & Adv Acc & \textbf{83.2} & \textbf{72.9} & \textbf{71.6} & \textbf{83.9} & \textbf{80.0} & \textbf{76.8} & \textbf{72.7} & \textbf{83.0} \\
 &  & Mixed Acc & \textbf{80.8} & \textbf{75.5} & \textbf{75.0} & \textbf{81.3} & \textbf{79.2} & \textbf{77.7} & \textbf{75.5} & \textbf{80.4} \\ \hline \hline
\multirow{12}{*}{{\begin{sideways}PointMLP\end{sideways}}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & 61.7 & 61.7 & 61.7 & 61.7 & 61.7 & 61.7 & 61.7 & 61.7 \\
 &  & Adv Acc & 51.5 & 43.1 & 35.0 & 54.7 & 40.4 & 42.5 & 34.9 & 58.1 \\
 &  & Mixed Acc & 56.6 & 52.4 & 48.3 & 58.1 & 51.1 & 51.2 & 48.3 & 59.9 \\ \cline{2-11} 
 & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \textbf{81.4} & \textbf{80.3} & \textbf{82.2} & \textbf{81.6} & \textbf{81.1} & \textbf{81.0} & \textbf{80.5} & \textbf{82.3} \\
 &  & Adv Acc & \textbf{79.5} & \textbf{76.2} & \textbf{74.0} & \textbf{78.3} & \textbf{81.3} & \textbf{77.2} & \textbf{73.5} & \textbf{79.5} \\
 &  & Mixed Acc & \textbf{80.4} & \textbf{78.2} & \textbf{78.1} & \textbf{80.0} & \textbf{81.2} & \textbf{79.1} & \textbf{77.0} & \textbf{80.9} \\ \cline{2-11} 
 & \multirow{3}{*}{IF-Def~\cite{wu2021ifdefense}} & Clean Acc & 74.5 & 74.1 & 75.2 & 74.7 & 73.3 & 73.8 & 74.2 & 75.0 \\
 &  & Adv Acc & 78.8 & 64.2 & 63.8 & 79.9 & 76.9 & 72.0 & 62.3 & 82.2 \\
 &  & Mixed Acc & 76.6 & 69.2 & 69.5 & 77.3 & 75.1 & 73.0 & 68.3 & 78.6 \\ \cline{2-11} 
 & \multirow{3}{*}{IF-Def+PST(Ours)} & Clean Acc & \textbf{77.4} & \textbf{74.8} & \textbf{76.5} & \textbf{77.8} & \textbf{77.4} & \textbf{77.6} & \textbf{75.2} & \textbf{78.3} \\
 &  & Adv Acc & \textbf{82.6} & \textbf{72.2} & \textbf{73.9} & \textbf{83.3} & \textbf{82.4} & \textbf{78.0} & \textbf{73.3} & \textbf{83.6} \\
 &  & Mixed Acc & \textbf{80.0} & \textbf{73.5} & \textbf{75.2} & \textbf{80.5} & \textbf{79.9} & \textbf{77.8} & \textbf{74.3} & \textbf{80.9} \\ \hline
\end{tabular}


==> sup_table/plain_acc.tex <==

\begin{tabular}{clcccccccc|cccccccc}
\hline
\multicolumn{2}{l}{\multirow{3}{*}{\textbf{}}} & \multicolumn{8}{c|}{Single Attack} & \multicolumn{8}{c}{Mixed Attack} \\ \cline{3-18} 
\multicolumn{2}{l}{} & \multicolumn{4}{c|}{\( l_\infty \)} & \multicolumn{4}{c|}{\( l_2 \)} & \multicolumn{4}{c|}{\( l_\infty \)} & \multicolumn{4}{c}{\( l_2 \)} \\ \cline{3-18} 
\multicolumn{2}{l}{} & C\&W & PGD & AdvPC & \multicolumn{1}{c|}{SI\_Adv} & C\&W & PGD & AdvPC & KNN & C\&W & PGD & AdvPC & \multicolumn{1}{c|}{SI\_Adv} & C\&W & PGD & AdvPC & KNN \\ \hline
\multirow{3}{*}{PCT} & Clean Acc & \textbf{93.7} & \textbf{93.7} & \textbf{93.7} & \multicolumn{1}{c|}{\textbf{93.7}} & \textbf{93.7} & \textbf{93.7} & \textbf{93.7} & \textbf{93.7} & \multicolumn{4}{c|}{\textbf{89.3}} & \multicolumn{4}{c}{\textbf{89.3}} \\
 & Adv Acc & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \multicolumn{1}{c|}{\textbf{27.6}} & \textbf{2.6} & \textbf{0.0} & \textbf{0.0} & \textbf{66.8} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \multicolumn{1}{c|}{\textbf{35.7}} & \textbf{2.2} & \textbf{0.0} & \textbf{0.0} & \textbf{70.3} \\
 & Mixed Acc & \textbf{46.9} & \textbf{46.9} & \textbf{46.9} & \multicolumn{1}{c|}{\textbf{60.7}} & \textbf{48.2} & \textbf{46.9} & \textbf{46.9} & \textbf{80.2} & \multicolumn{4}{c|}{\textbf{25.1}} & \multicolumn{4}{c}{\textbf{32.4}} \\ \hline \hline
\multirow{3}{*}{PointNet++} & Clean Acc & \textbf{92.9} & \textbf{92.9} & \textbf{92.9} & \multicolumn{1}{c|}{\textbf{92.9}} & \textbf{92.9} & \textbf{92.9} & \textbf{92.9} & \textbf{92.9} & \multicolumn{4}{c|}{\textbf{89.3}} & \multicolumn{4}{c}{\textbf{89.3}} \\
 & Adv Acc & \textbf{1.2} & \textbf{3.5} & \textbf{3.8} & \multicolumn{1}{c|}{\textbf{8.0}} & \textbf{1.7} & \textbf{14.1} & \textbf{3.8} & \textbf{42.8} & \textbf{0.8} & \textbf{0.0} & \textbf{12.5} & \multicolumn{1}{c|}{\textbf{20.4}} & \textbf{1.4} & \textbf{2.2} & \textbf{12.5} & \textbf{40.7} \\
 & Mixed Acc & \textbf{47.1} & \textbf{48.3} & \textbf{48.4} & \multicolumn{1}{c|}{\textbf{50.5}} & \textbf{47.3} & \textbf{53.5} & \textbf{48.4} & \textbf{67.9} & \multicolumn{4}{c|}{\textbf{24.5}} & \multicolumn{4}{c}{\textbf{29.3}} \\ \hline \hline
\multirow{3}{*}{CurveNet} & Clean Acc & \textbf{93.7} & \textbf{93.7} & \textbf{93.7} & \multicolumn{1}{c|}{\textbf{93.7}} & \textbf{93.7} & \textbf{93.7} & \textbf{93.7} & \textbf{93.7} & \multicolumn{4}{c|}{\textbf{90.7}} & \multicolumn{4}{c}{\textbf{90.7}} \\
 & Adv Acc & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \multicolumn{1}{c|}{\textbf{32.4}} & \textbf{3.9} & \textbf{3.1} & \textbf{0.0} & \textbf{70.7} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \multicolumn{1}{c|}{\textbf{25.7}} & \textbf{3.2} & \textbf{0.0} & \textbf{0.0} & \textbf{72.0} \\
 & Mixed Acc & \textbf{46.9} & \textbf{46.9} & \textbf{46.9} & \multicolumn{1}{c|}{\textbf{63.1}} & \textbf{48.9} & \textbf{48.5} & \textbf{46.9} & \textbf{82.2} & \multicolumn{4}{c|}{\textbf{23.2}} & \multicolumn{4}{c}{\textbf{33.2}} \\ \hline \hline
\multirow{3}{*}{PointNet} & Clean Acc & \textbf{91.5} & \textbf{91.5} & \textbf{91.5} & \multicolumn{1}{c|}{\textbf{91.5}} & \textbf{91.5} & \textbf{91.5} & \textbf{91.5} & \textbf{91.5} & \multicolumn{4}{c|}{\textbf{85.6}} & \multicolumn{4}{c}{\textbf{85.6}} \\
 & Adv Acc & \textbf{2.3} & \textbf{1.7} & \textbf{2.2} & \multicolumn{1}{c|}{\textbf{47.9}} & \textbf{2.6} & \textbf{28.6} & \textbf{2.2} & \textbf{54.4} & \textbf{1.2} & \textbf{0.0} & \textbf{10.7} & \multicolumn{1}{c|}{\textbf{62.2}} & \textbf{1.8} & \textbf{31.0} & \textbf{10.7} & \textbf{61.4} \\
 & Mixed Acc & \textbf{46.9} & \textbf{46.6} & \textbf{46.9} & \multicolumn{1}{c|}{\textbf{69.7}} & \textbf{47.1} & \textbf{60.1} & \textbf{46.9} & \textbf{73.0} & \multicolumn{4}{c|}{\textbf{31.9}} & \multicolumn{4}{c}{\textbf{38.2}} \\ \hline \hline
\multirow{3}{*}{DGCNN} & Clean Acc & \textbf{93.7} & \textbf{93.7} & \textbf{93.7} & \multicolumn{1}{c|}{\textbf{93.7}} & \textbf{93.7} & \textbf{93.7} & \textbf{93.7} & \textbf{93.7} & \multicolumn{4}{c|}{\textbf{88.1}} & \multicolumn{4}{c}{\textbf{88.1}} \\
 & Adv Acc & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \multicolumn{1}{c|}{\textbf{0.0}} & \textbf{2.5} & \textbf{0.0} & \textbf{0.4} & \textbf{52.7} & \textbf{0.0} & \textbf{0.0} & \textbf{0.2} & \multicolumn{1}{c|}{\textbf{0.4}} & \textbf{2.2} & \textbf{0.0} & \textbf{1.2} & \textbf{55.5} \\
 & Mixed Acc & \textbf{46.9} & \textbf{46.9} & \textbf{46.9} & \multicolumn{1}{c|}{\textbf{46.9}} & \textbf{48.1} & \textbf{46.9} & \textbf{47.1} & \textbf{73.2} & \multicolumn{4}{c|}{\textbf{17.7}} & \multicolumn{4}{c}{\textbf{29.5}} \\ \hline \hline
\multirow{3}{*}{PointMLP} & Clean Acc & \textbf{94.9} & \textbf{94.9} & \textbf{94.9} & \multicolumn{1}{c|}{\textbf{94.9}} & \textbf{94.9} & \textbf{94.9} & \textbf{94.9} & \textbf{94.9} & \multicolumn{4}{c|}{\textbf{91.1}} & \multicolumn{4}{c}{\textbf{91.1}} \\
 & Adv Acc & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \multicolumn{1}{c|}{\textbf{41.8}} & \textbf{2.0} & \textbf{0.2} & \textbf{0.0} & \textbf{35.6} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \multicolumn{1}{c|}{\textbf{48.6}} & \textbf{1.2} & \textbf{0.0} & \textbf{0.0} & \textbf{43.6} \\
 & Mixed Acc & \textbf{47.5} & \textbf{47.5} & \textbf{47.5} & \multicolumn{1}{c|}{\textbf{68.4}} & \textbf{48.5} & \textbf{47.6} & \textbf{47.5} & \textbf{65.3} & \multicolumn{4}{c|}{\textbf{27.9}} & \multicolumn{4}{c}{\textbf{27.2}} \\ \hline
\end{tabular}


==> sup_table/plain_acc_scan.tex <==

\begin{tabular}{clccclcccc|ccclcccc}
\hline
\multicolumn{2}{l}{\multirow{3}{*}{\textbf{}}} & \multicolumn{8}{c|}{Single Attack} & \multicolumn{8}{c}{Mixed Attack} \\ \cline{3-18} 
\multicolumn{2}{l}{} & \multicolumn{4}{c|}{\( l_\infty \)} & \multicolumn{4}{c|}{\( l_2 \)} & \multicolumn{4}{c|}{\( l_\infty \)} & \multicolumn{4}{c}{\( l_2 \)} \\ \cline{3-18} 
\multicolumn{2}{l}{} & C\&W & PGD & \multicolumn{2}{c|}{AdvPC} & C\&W & PGD & AdvPC & KNN & C\&W & PGD & \multicolumn{2}{c|}{AdvPC} & C\&W & PGD & AdvPC & KNN \\ \hline
\multirow{3}{*}{PCT} & Clean Acc & \textbf{78.4} & \textbf{78.4} & \multicolumn{2}{c|}{\textbf{78.4}} & \textbf{78.4} & \textbf{78.4} & \textbf{78.4} & \textbf{78.4} & \multicolumn{4}{c|}{\textbf{75.5}} & \multicolumn{4}{c}{\textbf{82.4}} \\
 & Adv Acc & \textbf{0.0} & \textbf{0.0} & \multicolumn{2}{c|}{\textbf{0.0}} & \textbf{4.8} & \textbf{0.0} & \textbf{0.0} & \textbf{25.3} & \textbf{0.0} & \textbf{0.0} & \multicolumn{2}{c|}{\textbf{0.0}} & \textbf{4.3} & \textbf{0.0} & \textbf{0.0} & \textbf{23.1} \\
 & Mixed Acc & \textbf{39.2} & \textbf{39.2} & \multicolumn{2}{c|}{\textbf{39.2}} & \textbf{41.6} & \textbf{39.2} & \textbf{39.2} & \textbf{51.9} & \multicolumn{4}{c|}{\textbf{18.8}} & \multicolumn{4}{c}{\textbf{22.0}} \\ \hline \hline
\multirow{3}{*}{PointNet++} & Clean Acc & \textbf{80.1} & \textbf{80.1} & \multicolumn{2}{c|}{\textbf{80.1}} & \textbf{80.1} & \textbf{80.1} & \textbf{80.1} & \textbf{80.1} & \multicolumn{4}{c|}{\textbf{80.1}} & \multicolumn{4}{c}{\textbf{81.7}} \\
 & Adv Acc & \textbf{0.0} & \textbf{0.0} & \multicolumn{2}{c|}{\textbf{0.1}} & \textbf{2.4} & \textbf{4.5} & \textbf{1.3} & \textbf{16.4} & \textbf{0.0} & \textbf{0.0} & \multicolumn{2}{c|}{\textbf{0.1}} & \textbf{1.3} & \textbf{5.2} & \textbf{0.8} & \textbf{11.9} \\
 & Mixed Acc & \textbf{40.1} & \textbf{40.1} & \multicolumn{2}{c|}{\textbf{40.1}} & \textbf{41.3} & \textbf{42.3} & \textbf{40.7} & \textbf{48.3} & \multicolumn{4}{c|}{\textbf{20.0}} & \multicolumn{4}{c}{\textbf{20.1}} \\ \hline \hline
\multirow{3}{*}{CurveNet} & Clean Acc & \textbf{78.7} & \textbf{78.7} & \multicolumn{2}{c|}{\textbf{78.7}} & \textbf{78.7} & \textbf{78.7} & \textbf{78.7} & \textbf{78.7} & \multicolumn{4}{c|}{\textbf{77.2}} & \multicolumn{4}{c}{\textbf{81.7}} \\
 & Adv Acc & \textbf{0.0} & \textbf{0.0} & \multicolumn{2}{c|}{\textbf{0.2}} & \textbf{3.9} & \textbf{1.4} & \textbf{0.6} & \textbf{34.7} & \textbf{0.0} & \textbf{0.0} & \multicolumn{2}{c|}{\textbf{0.2}} & \textbf{2.7} & \textbf{1.2} & \textbf{1.8} & \textbf{29.8} \\
 & Mixed Acc & \textbf{39.4} & \textbf{39.4} & \multicolumn{2}{c|}{\textbf{39.5}} & \textbf{41.3} & \textbf{40.1} & \textbf{39.6} & \textbf{56.8} & \multicolumn{4}{c|}{\textbf{19.3}} & \multicolumn{4}{c}{\textbf{23.4}} \\ \hline
\end{tabular}


==> table/bk_tables.tex <==


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[!tbp]
  \centering
  \caption{Evaluation of robustness against white-box attacks on ModelNet40 dataset. Both Single Attack and Mixed Attack are reported on five types of adversarial attacks.}
  \resizebox{0.99\linewidth}{!}{
\begin{tabular}{|cll|cccccccc|cccccccc|}
\hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{3}{|c|}{\cellcolor[HTML]{FFFFFF}}                                                                                                                                                                                   & \multicolumn{8}{c|}{\cellcolor[HTML]{FFFFFF}Single Attack}                                                                                                                                                                                                                                                                                                                                                                                               & \multicolumn{8}{c|}{\cellcolor[HTML]{FFFFFF}Mixed Attack}                                                                                                                                                                                                                                                                                                                                                                                                \\ \cline{4-19} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{3}{|c|}{\cellcolor[HTML]{FFFFFF}}                                                                                                                                                                                   & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}\( l_\infty \)}                                                                                                                                                                                                    & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}\( l_2 \)}                                                                                                                                                      & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}\( l_\infty \)}                                                                                                                                                                                                    & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}\( l_2 \)}                                                                                                                                                      \\ \cline{4-19} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{3}{|c|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}}}                                                                                                                                                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}C\&W}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}PGD}           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}AdvPC}         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}SI\_Adv}       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}C\&W}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}PGD}           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}AdvPC}         & KNN           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}C\&W}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}PGD}           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}AdvPC}         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}SI\_Adv}       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}C\&W}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}PGD}           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}AdvPC}         & KNN           \\ \hline
\rowcolor[HTML]{FBDAD7} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.4}          & 80.4          & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}72.3}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}72.3}                                                                                                                                                    \\ \cline{3-19} 
\rowcolor[HTML]{FEF2CD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}77.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}69.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}63.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}77.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}75.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}57.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}62.8}          & 79.2          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}74.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}71.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}76.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}71.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}74.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}54.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}76.0}          & \textbf{76.1} \\ \cline{3-19} 
\rowcolor[HTML]{D9E7FD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}Pt. DP}}                                                         & Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}79.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}75.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}71.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}78.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}77.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}69.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}71.6}          & 79.8          & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}73.2}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}70.5}                                                                                                                                                    \\ \cline{2-19} 
\rowcolor[HTML]{FBDAD7} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.7}} & \textbf{85.1} & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{78.2}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{80.4}}                                                                                                                                           \\ \cline{3-19} 
\rowcolor[HTML]{FEF2CD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{82.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{77.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{75.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{82.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{82.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{72.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{74.8}} & \textbf{84.3} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{84.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{82.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{89.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{73.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{79.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{77.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{89.5}} & 75.9          \\ \cline{3-19} 
\rowcolor[HTML]{D9E7FD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}Pt. DP+\\ S.T. (Ours)\end{tabular}}}  & Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{83.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{80.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{83.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{83.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{78.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.3}} & \textbf{84.7} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.6}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{80.5}}                                                                                                                                           \\ \cline{2-19} 
\rowcolor[HTML]{FBDAD7} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}79.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.2}          & 78.4          & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}81.8}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}82.2}                                                                                                                                           \\ \cline{3-19} 
\rowcolor[HTML]{FEF2CD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}83.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}54.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}54.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}82.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}82.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}69.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}53.9}          & 84.8          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}80.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}55.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}65.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{78.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}77.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}77.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}65.7}          & \textbf{80.3} \\ \cline{3-19} 
\rowcolor[HTML]{D9E7FD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}IF-Def.}}                                                        & Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}80.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}66.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}67.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}80.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}80.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}74.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}66.1}          & 81.6          & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}72.5}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}76.7}                                                                                                                                                    \\ \cline{2-19} 
\rowcolor[HTML]{FBDAD7} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{82.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{80.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{80.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{81.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{80.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{79.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{79.8}} & \textbf{81.7} & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.9}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{85.3}}                                                                                                                                           \\ \cline{3-19} 
\rowcolor[HTML]{FEF2CD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{84.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{67.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{67.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{85.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{84.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{76.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{67.0}} & \textbf{86.7} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{79.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{71.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{83.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}77.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{80.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{79.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{84.4}} & 77.3          \\ \cline{3-19} 
\rowcolor[HTML]{D9E7FD} 
\multicolumn{1}{|c|}{\multirow{-12}{*}{\cellcolor[HTML]{FFFFFF}\textbf{Curvenet}}}   & \multicolumn{1}{l|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}IF-Def.\\ +S.T. (Ours)\end{tabular}}} & Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{82.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{74.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{74.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{83.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{82.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{78.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{73.4}} & \textbf{84.2} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.2}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.4}}                                                                                                                                           \\ \hline
\rowcolor[HTML]{FBDAD7} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.1}          & 78.1          & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}70.3}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}70.3}                                                                                                                                                    \\ \cline{3-19} 
\rowcolor[HTML]{FEF2CD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}74.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}66.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}62.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}71.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}67.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}69.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}62.0}          & 76.9          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}72.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}70.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}74.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}67.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}65.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}68.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}74.0}          & 69.3          \\ \cline{3-19} 
\rowcolor[HTML]{D9E7FD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}Pt. DP}}                                                         & Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}76.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}72.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}70.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}74.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}72.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}73.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}70.1}          & 77.5          & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}71.0}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}69.7}                                                                                                                                                    \\ \cline{2-19} 
\rowcolor[HTML]{FBDAD7} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{81.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.6}} & \textbf{83.8} & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{75.0}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{75.8}}                                                                                                                                           \\ \cline{3-19} 
\rowcolor[HTML]{FEF2CD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}81.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{79.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{76.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}81.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}80.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{78.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{76.0}} & 82.9          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{80.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{85.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{91.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{74.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{78.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{81.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{91.3}} & \textbf{75.7} \\ \cline{3-19} 
\rowcolor[HTML]{D9E7FD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}Pt. DP\\ +S.T. (Ours)\end{tabular}}}  & Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{82.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{82.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.8}} & \textbf{83.4} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.3}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{80.6}}                                                                                                                                           \\ \cline{2-19} 
\rowcolor[HTML]{FBDAD7} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}79.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}79.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}79.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}79.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}79.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}79.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}79.2}          & 79.3          & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}84.0}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.6}}                                                                                                                                           \\ \cline{3-19} 
\rowcolor[HTML]{FEF2CD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}83.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}73.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}70.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}83.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}81.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}77.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}71.1}          & 83.9          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}79.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}75.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}82.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{79.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}74.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}83.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}79.5}          & \textbf{78.5} \\ \cline{3-19} 
\rowcolor[HTML]{D9E7FD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}IF-Def.}}                                                        & Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}81.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}76.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}74.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}81.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}80.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}78.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}75.2}          & 81.6          & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}80.0}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}80.1}                                                                                                                                                    \\ \cline{2-19} 
\rowcolor[HTML]{FBDAD7} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{82.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{81.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{80.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{81.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{80.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{81.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{81.3}} & \textbf{81.0} & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.1}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.1}}                                                                                                                                           \\ \cline{3-19} 
\rowcolor[HTML]{FEF2CD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{84.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{77.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{76.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{85.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{83.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{80.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{77.3}} & \textbf{84.7} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{79.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{84.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{89.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}78.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{78.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{86.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{88.7}} & 78.3          \\ \cline{3-19} 
\rowcolor[HTML]{D9E7FD} 
\multicolumn{1}{|c|}{\multirow{-12}{*}{\cellcolor[HTML]{FFFFFF}\textbf{PointNet\texttt{++}}}} & \multicolumn{1}{l|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}IF-Def.\\ +S.T. (Ours)\end{tabular}}} & Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{83.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{78.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{83.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.3}} & \textbf{82.8} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{83.2}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{83.1}}                                                                                                                                           \\ \hline
\rowcolor[HTML]{FBDAD7} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}81.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}81.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}81.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}81.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}81.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}81.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}81.2}          & 81.2          & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}73.9}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}73.9}                                                                                                                                                    \\ \cline{3-19} 
\rowcolor[HTML]{FEF2CD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}77.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}70.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}64.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}76.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}75.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}60.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}65.3}          & 80.4          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}71.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}72.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}81.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}74.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}70.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}58.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}81.1}          & 78.1          \\ \cline{3-19} 
\rowcolor[HTML]{D9E7FD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}Pt. DP}}                                                         & Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}79.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}75.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}72.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}78.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}78.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}70.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}73.2}          & 80.8          & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}74.5}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}72.3}                                                                                                                                                    \\ \cline{2-19} 
\rowcolor[HTML]{FBDAD7} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{82.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{81.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.9}} & \textbf{84.6} & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}82.3}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.9}}                                                                                                                                           \\ \cline{3-19} 
\rowcolor[HTML]{FEF2CD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}80.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{75.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{71.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}82.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}80.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{71.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{72.0}} & 83.0          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{85.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{71.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{85.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}79.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{81.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{78.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{84.2}} & 77.9          \\ \cline{3-19} 
\rowcolor[HTML]{D9E7FD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}Pt. DP\\ +S.T. (Ours)\end{tabular}}}  & Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}81.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{77.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}82.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{82.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{77.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{78.0}} & \textbf{83.8} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.4}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.3}}                                                                                                                                           \\ \cline{2-19} 
\rowcolor[HTML]{FBDAD7} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}81.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}81.3}          & 80.4          & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.6}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}82.4}                                                                                                                                                    \\ \cline{3-19} 
\rowcolor[HTML]{FEF2CD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}83.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}60.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}60.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}84.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}83.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}70.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}59.7}          & \textbf{86.6} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}78.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}61.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}74.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{80.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}78.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}73.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}74.2}          & \textbf{79.1} \\ \cline{3-19} 
\rowcolor[HTML]{D9E7FD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}IF-Def.}}                                                        & Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}81.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}70.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}71.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}82.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}82.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}75.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}70.5}          & \textbf{83.5} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}75.7}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}77.5}                                                                                                                                                    \\ \cline{2-19} 
\rowcolor[HTML]{FBDAD7} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{80.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{82.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{82.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{82.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{82.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{81.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{81.9}} & \textbf{80.4} & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}82.3}                                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.9}}                                                                                                                                           \\ \cline{3-19} 
\rowcolor[HTML]{FEF2CD} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                                                 & Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{83.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{69.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{67.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{85.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{84.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{75.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{69.6}} & 84.7          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{85.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{71.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{85.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}79.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{81.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{78.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{84.2}} & 77.9          \\ \cline{3-19} 
\rowcolor[HTML]{D9E7FD} 
\multicolumn{1}{|c|}{\multirow{-12}{*}{\cellcolor[HTML]{FFFFFF}\textbf{PCT}}}        & \multicolumn{1}{l|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}IF-Def.\\ +S.T. (Ours)\end{tabular}}} & Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{75.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{75.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{83.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{83.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{78.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{75.8}} & 82.5          & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.4}}                                                                                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.3}}                                                                                                                                           \\ \hline
\end{tabular}
    }
  \label{tab:ModelNet40_white}%
\end{table}%




% Table generated by Excel2LaTeX from sheet 'ScanObjectNN'
\begin{table}[!tbp]
  \centering
  \caption{Evaluation of robustness against white-box attacks on ScanObjectNN dataset. Both Single Attack and Mixed Attack are reported on five types of white-box adversarial attacks.}
    \resizebox{0.99\linewidth}{!}{
\begin{tabular}{|cll|ccccccc|ccccccc|}
\hline
\multicolumn{3}{|l|}{}                                                                                                                                                                                 & \multicolumn{7}{c|}{Single Attack}                                                                                                                                                                                                                                                                                                                                                                                  & \multicolumn{7}{c|}{Mixed Attack}                                                                                                                                                                                                                                                                                                                                                                                   \\ \cline{4-17} 
\multicolumn{3}{|l|}{}                                                                                                                                                                                 & \multicolumn{3}{c|}{\( l_\infty \)
}                                                                                                                                                               & \multicolumn{4}{c|}{\( l_2 \)}                                                                                                                                                                                                      & \multicolumn{3}{c|}{\( l_\infty \)}                                                                                                                                                               & \multicolumn{4}{c|}{\( l_2 \)}                                                                                                                                                                                                      \\ \cline{4-17} 
\multicolumn{3}{|l|}{\multirow{-3}{*}{}}                                                                                                                                                               & \multicolumn{1}{c|}{C\&W}                                  & \multicolumn{1}{c|}{PGD}                                   & \multicolumn{1}{c|}{AdvPC}                                 & \multicolumn{1}{c|}{C\&W}                                  & \multicolumn{1}{c|}{PGD}                                   & \multicolumn{1}{c|}{AdvPC}                                 & KNN                                   & \multicolumn{1}{c|}{C\&W}                                  & \multicolumn{1}{c|}{PGD}                                   & \multicolumn{1}{c|}{AdvPC}                                 & \multicolumn{1}{c|}{C\&W}                                  & \multicolumn{1}{c|}{PGD}                                   & \multicolumn{1}{c|}{AdvPC}                                 & KNN                                   \\ \hline
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}45.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}45.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}45.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}45.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}45.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}45.0}          & \cellcolor[HTML]{FBDAD7}45.0          & \multicolumn{3}{c|}{\cellcolor[HTML]{FBDAD7}42.3}                                                                                                                                    & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}42.8}                                                                                                                                                                            \\ \cline{3-17} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}34.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}23.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}21.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}33.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}24.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}46.8}          & \cellcolor[HTML]{FEF2CD}45.8          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}34.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}22.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}27.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}38.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}21.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}50.1}          & \cellcolor[HTML]{FEF2CD}36.8          \\ \cline{3-17} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{\multirow{-3}{*}{Pt. DP}}                                                        & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}40.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}34.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}33.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}39.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}34.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}45.9}          & \cellcolor[HTML]{D9E7FD}45.4          & \multicolumn{3}{c|}{\cellcolor[HTML]{D9E7FD}31.6}                                                                                                                                    & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}37.8}                                                                                                                                                                            \\ \cline{2-17} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{57.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{58.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{58.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{58.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{58.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{59.7}} & \cellcolor[HTML]{FBDAD7}\textbf{59.4} & \multicolumn{3}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{58.7}}                                                                                                                           & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{61.6}}                                                                                                                                                                   \\ \cline{3-17} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{54.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{44.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{41.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{53.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{44.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{59.8}} & \cellcolor[HTML]{FEF2CD}\textbf{60.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{54.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{45.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{41.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{54.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{47.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{56.1}} & \cellcolor[HTML]{FEF2CD}\textbf{50.9} \\ \cline{3-17} 
\multicolumn{1}{|c|}{\multirow{-6}{*}{\textbf{Curvenet}}}   & \multicolumn{1}{l|}{\multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}Pt. DP\\ +S.T. (Ours)\end{tabular}}} & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{56.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{51.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{49.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{55.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{51.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{59.8}} & \cellcolor[HTML]{D9E7FD}\textbf{59.7} & \multicolumn{3}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{49.7}}                                                                                                                           & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{54.2}}                                                                                                                                                                   \\ \hline
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.4}          & \cellcolor[HTML]{FBDAD7}47.4          & \multicolumn{3}{c|}{\cellcolor[HTML]{FBDAD7}42.4}                                                                                                                                    & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}57.2}                                                                                                                                                                            \\ \cline{3-17} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}37.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}21.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}16.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}27.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}31.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}47.0}          & \cellcolor[HTML]{FEF2CD}47.0          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}40.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}18.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}18.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}27.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}21.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}53.1}          & \cellcolor[HTML]{FEF2CD}44.2          \\ \cline{3-17} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{\multirow{-3}{*}{Pt. DP}}                                                        & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}42.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}34.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}32.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}27.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}39.4}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}47.2}          & \cellcolor[HTML]{D9E7FD}47.2          & \multicolumn{3}{c|}{\cellcolor[HTML]{D9E7FD}29.8}                                                                                                                                    & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}40.7}                                                                                                                                                                            \\ \cline{2-17} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{54.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{57.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{54.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{56.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{56.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{57.5}} & \cellcolor[HTML]{FBDAD7}\textbf{57.1} & \multicolumn{3}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{54.4}}                                                                                                                           & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{62.9}}                                                                                                                                                                   \\ \cline{3-17} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{48.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{47.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{41.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{48.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{49.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{58.1}} & \cellcolor[HTML]{FEF2CD}\textbf{57.6} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{51.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{48.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{44.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{45.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{47.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{53.7}} & \cellcolor[HTML]{FEF2CD}\textbf{64.9} \\ \cline{3-17} 
\multicolumn{1}{|c|}{\multirow{-6}{*}{\textbf{PointNet\texttt{++}}}} & \multicolumn{1}{l|}{\multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}Pt. DP\\ +S.T. (Ours)\end{tabular}}} & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{51.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{52.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{48.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{52.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{52.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{57.8}} & \cellcolor[HTML]{D9E7FD}\textbf{57.4} & \multicolumn{3}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{49.4}}                                                                                                                           & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{54.8}}                                                                                                                                                                   \\ \hline
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.5}          & \cellcolor[HTML]{FBDAD7}47.5          & \multicolumn{3}{c|}{\cellcolor[HTML]{FBDAD7}49.0}                                                                                                                                    & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}47.9}                                                                                                                                                                            \\ \cline{3-17} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}39.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}24.8}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}22.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}35.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}23.1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}49.7}          & \cellcolor[HTML]{FEF2CD}47.0          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}52.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}15.6}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}12.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}38.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}19.9}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}47.7}          & \cellcolor[HTML]{FEF2CD}38.8          \\ \cline{3-17} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{\multirow{-3}{*}{Pt. DP}}                                                        & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}43.7}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}36.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}35.2}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}41.5}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}35.3}          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}48.6}          & \cellcolor[HTML]{D9E7FD}47.3          & \multicolumn{3}{c|}{\cellcolor[HTML]{D9E7FD}32.3}                                                                                                                                    & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}38.5}                                                                                                                                                                            \\ \cline{2-17} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{54.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{53.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{54.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{54.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{54.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{56.0}} & \cellcolor[HTML]{FBDAD7}\textbf{56.3} & \multicolumn{3}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{52.1}}                                                                                                                           & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{56.9}}                                                                                                                                                                   \\ \cline{3-17} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{48.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{40.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{39.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{50.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{38.6}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{58.4}} & \cellcolor[HTML]{FEF2CD}\textbf{56.9} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{71.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{30.3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{23.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{53.8}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{39.4}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{56.9}} & \cellcolor[HTML]{FEF2CD}\textbf{54.9} \\ \cline{3-17} 
\multicolumn{1}{|c|}{\multirow{-6}{*}{\textbf{PCT}}}        & \multicolumn{1}{l|}{\multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}Pt. DP\\ +S.T. (Ours)\end{tabular}}} & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{51.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{47.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{47.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{52.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{46.5}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{57.2}} & \cellcolor[HTML]{D9E7FD}\textbf{56.6} & \multicolumn{3}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{44.3}}                                                                                                                           & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{52.4}}                                                                                                                                                                   \\ \hline
\end{tabular}
    }
  \label{tab:ScanObjectNN_white}%
\end{table}%



% Table generated by Excel2LaTeX from sheet 'AdaptiveAttack'
\begin{table}[tbp]
  \centering
  \vspace{-0.5cm}
  \caption{Evaluation of robustness against adaptive attacks on ModelNet40 and ScanObjectNN datasets under Single Attack protocol.}
      \resizebox{0.9\linewidth}{!}{
\begin{tabular}{|cll|cccccccc|cccccccc|}
\hline
\multicolumn{3}{|l|}{}                                                                                                                                                                                 & \multicolumn{8}{c|}{ModelNet40}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & \multicolumn{8}{c|}{ScanObjectNN}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           \\ \cline{4-19} 
\multicolumn{3}{|l|}{}                                                                                                                                                                                 & \multicolumn{4}{c|}{\( l_\infty \)}                                                                                                                                                                                                                                                                                                & \multicolumn{4}{c|}{\( l_2 \)}                                                                                                                                                                                                                                                                          & \multicolumn{4}{c|}{\( l_\infty \)}                                                                                                                                                                                                                                                                                                & \multicolumn{4}{c|}{\( l_2 \)}                                                                                                                                                                                                                                                                          \\ \cline{4-19} 
\multicolumn{3}{|l|}{\multirow{-3}{*}{}}                                                                                                                                                               & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BPDA-\\ PGD\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}EOT-\\ AutoAttack\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}PGD-\\ Latent\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}AdvPC-\\ Latent\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BPDA-\\ PGD\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}EOT-\\ AutoAttack\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}PGD-\\ Latent\end{tabular}} & \begin{tabular}[c]{@{}c@{}}AdvPC-\\ Latent\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BPDA-\\ PGD\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}EOT-\\ AutoAttack\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}PGD-\\ Latent\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}AdvPC-\\ Latent\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BPDA-\\ PGD\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}EOT-\\ AutoAttack\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}PGD-\\ Latent\end{tabular}} & \begin{tabular}[c]{@{}c@{}}AdvPC-\\ Latent\end{tabular} \\ \hline
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.4}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.4}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.4}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.4}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.4}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.4}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}80.4}                          & \cellcolor[HTML]{FBDAD7}80.4                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}45.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}45.0}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}45.0}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}45.0}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}45.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}45.0}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}45.0}                          & \cellcolor[HTML]{FBDAD7}45.0                            \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}65.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}67.7}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}65.4}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}49.7}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}72.2}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}77.1}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}87.5}                          & \cellcolor[HTML]{FEF2CD}79.9                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}25.6}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}25.2}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}34.0}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}22.9}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}38.9}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}43.4}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}55.5}                          & \cellcolor[HTML]{FEF2CD}47.7                            \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{\multirow{-3}{*}{Pt. DP}}                                                        & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}72.7}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}74.1}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}72.9}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}65.1}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}76.3}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}78.7}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}83.9}                          & \cellcolor[HTML]{D9E7FD}80.1                            & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}35.4}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}35.1}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}39.5}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}34.0}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}42.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}44.2}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}50.3}                          & \cellcolor[HTML]{D9E7FD}46.3                            \\ \cline{2-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.2}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.2}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.3}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.4}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{85.0}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.2}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.3}}                 & \cellcolor[HTML]{FBDAD7}\textbf{85.0}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{58.2}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{58.6}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{57.6}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{58.0}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{61.1}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{59.9}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{59.9}}                 & \cellcolor[HTML]{FBDAD7}\textbf{58.7}                   \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{78.1}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{76.9}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{85.1}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{63.6}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{79.6}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{82.4}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{89.4}}                 & \cellcolor[HTML]{FEF2CD}\textbf{84.2}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{49.0}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{44.9}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{53.7}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{37.9}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{57.7}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{59.4}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{65.6}}                 & \cellcolor[HTML]{FEF2CD}\textbf{59.6}                   \\ \cline{3-19} 
\multicolumn{1}{|c|}{\multirow{-6}{*}{\textbf{CurveNet}}}   & \multicolumn{1}{l|}{\multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}Pt. DP\\ +S.T. (Ours)\end{tabular}}} & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.1}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{80.0}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{84.7}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{74.0}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{82.3}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{83.3}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{86.8}}                 & \cellcolor[HTML]{D9E7FD}\textbf{84.6}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{53.6}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{51.8}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{55.6}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{48.0}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{59.4}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{59.6}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{62.7}}                 & \cellcolor[HTML]{D9E7FD}\textbf{59.1}                   \\ \hline
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.0}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.0}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.0}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.0}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}78.0}                          & \cellcolor[HTML]{FBDAD7}78.0                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.4}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.4}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.4}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.4}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.4}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.4}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.4}                          & \cellcolor[HTML]{FBDAD7}47.4                            \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}64.5}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}66.1}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}45.7}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}38.9}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}68.8}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}74.5}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}82.7}                          & \cellcolor[HTML]{FEF2CD}77.4                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}17.6}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}19.7}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}29.7}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}16.5}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}28.1}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}44.9}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}50.6}                          & \cellcolor[HTML]{FEF2CD}47.5                            \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{\multirow{-3}{*}{Pt. DP}}                                                        & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}71.3}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}72.1}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}61.9}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}58.5}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}73.4}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}76.3}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}80.3}                          & \cellcolor[HTML]{D9E7FD}77.7                            & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}32.5}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}33.6}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}38.6}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}31.9}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}37.8}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}46.1}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}49.0}                          & \cellcolor[HTML]{D9E7FD}47.5                            \\ \cline{2-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{82.7}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.9}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{82.9}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{82.4}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.3}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.0}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.0}}                 & \cellcolor[HTML]{FBDAD7}\textbf{83.2}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{57.0}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{56.5}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{56.9}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{56.0}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{56.6}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{57.2}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{57.8}}                 & \cellcolor[HTML]{FBDAD7}\textbf{56.0}                   \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{80.4}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{78.8}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{78.7}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{64.2}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{79.2}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{81.7}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{89.0}}                 & \cellcolor[HTML]{FEF2CD}\textbf{84.0}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{47.2}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{45.4}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{54.3}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{39.2}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{49.7}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{57.4}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{63.8}}                 & \cellcolor[HTML]{FEF2CD}\textbf{59.0}                   \\ \cline{3-19} 
\multicolumn{1}{|c|}{\multirow{-6}{*}{\textbf{PointNet\texttt{++}~}}} & \multicolumn{1}{l|}{\multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}Pt. DP\\ +S.T. (Ours)\end{tabular}}} & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.5}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.4}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{80.8}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{73.3}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.3}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{82.3}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{86.0}}                 & \cellcolor[HTML]{D9E7FD}\textbf{83.6}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{52.1}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{51.0}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{55.6}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{47.6}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{53.1}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{57.3}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{60.8}}                 & \cellcolor[HTML]{D9E7FD}\textbf{57.5}                   \\ \hline
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}81.2}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}81.2}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}81.2}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}81.2}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}81.2}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}81.2}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}81.2}                          & \cellcolor[HTML]{FBDAD7}81.2                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.5}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.5}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.5}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.5}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.5}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.5}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}47.5}                          & \cellcolor[HTML]{FBDAD7}47.5                            \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}69.1}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}70.5}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}68.0}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}50.3}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}72.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}77.5}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}88.3}                          & \cellcolor[HTML]{FEF2CD}80.6                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}28.8}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}25.2}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}36.1}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}22.9}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}38.2}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}46.3}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}56.5}                          & \cellcolor[HTML]{FEF2CD}49.7                            \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{\multirow{-3}{*}{Pt. DP}}                                                        & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}75.2}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}75.8}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}74.6}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}65.8}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}76.6}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}79.3}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}84.7}                          & \cellcolor[HTML]{D9E7FD}80.9                            & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}38.2}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}36.4}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}41.8}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}35.2}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}42.9}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}46.9}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}52.1}                          & \cellcolor[HTML]{D9E7FD}48.6                            \\ \cline{2-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{82.6}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.0}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.3}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.8}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{83.1}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{82.2}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{84.6}}                 & \cellcolor[HTML]{FBDAD7}\textbf{81.3}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{55.4}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{53.2}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{51.0}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{53.5}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{55.1}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{56.9}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{57.0}}                 & \cellcolor[HTML]{FBDAD7}\textbf{56.7}                   \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FEF2CD}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{76.0}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{76.6}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{81.9}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{59.8}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{77.0}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{79.6}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{87.7}}                 & \cellcolor[HTML]{FEF2CD}\textbf{81.2}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{46.9}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{42.4}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{44.3}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{39.1}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{50.9}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{55.3}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{63.7}}                 & \cellcolor[HTML]{FEF2CD}\textbf{58.8}                   \\ \cline{3-19} 
\multicolumn{1}{|c|}{\multirow{-6}{*}{\textbf{PCT}}}        & \multicolumn{1}{l|}{\multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}Pt. DP\\ +S.T. (Ours)\end{tabular}}} & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.3}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{80.3}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{83.1}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{71.8}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{80.0}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.0}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{86.2}}                 & \cellcolor[HTML]{D9E7FD}\textbf{81.3}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{51.2}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{47.8}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{47.6}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{46.3}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{53.0}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{56.1}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{60.3}}                 & \cellcolor[HTML]{D9E7FD}\textbf{57.7}                   \\ \hline
\end{tabular}
    }
    \vspace{-0.5cm}
  \label{tab:adaptive_single}%
\end{table}%



\begin{table}[htbp]
\centering
  \caption{Evaluation of robustness against adaptive attacks on ModelNet40 and ScanObjectNN datasets under Mixed Attack protocol.}
      \resizebox{0.99\linewidth}{!}{
\begin{tabular}{|cll|cccccccc|cccccccc|}
\hline
\multicolumn{3}{|l|}{}                                                                                                                                                                                 & \multicolumn{8}{c|}{ModelNet40}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & \multicolumn{8}{c|}{ScanObjectNN}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           \\ \cline{4-19} 
\multicolumn{3}{|l|}{}                                                                                                                                                                                 & \multicolumn{4}{c|}{\( l_\infty \)}                                                                                                                                                                                                                                                                                                & \multicolumn{4}{c|}{\( l_2 \)}                                                                                                                                                                                                                                                                          & \multicolumn{4}{c|}{\( l_\infty \)}                                                                                                                                                                                                                                                                                                & \multicolumn{4}{c|}{\( l_2 \)}                                                                                                                                                                                                                                                                          \\ \cline{4-19} 
\multicolumn{3}{|l|}{\multirow{-3}{*}{}}                                                                                                                                                               & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BPDA-\\ PGD\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}EOT-\\ AutoAttack\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}PGD-\\ Latent\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}AdvPC-\\ Latent\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BPDA-\\ PGD\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}EOT-\\ AutoAttack\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}PGD-\\ Latent\end{tabular}} & \begin{tabular}[c]{@{}c@{}}AdvPC-\\ Latent\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BPDA-\\ PGD\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}EOT-\\ AutoAttack\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}PGD-\\ Latent\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}AdvPC-\\ Latent\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BPDA-\\ PGD\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}EOT-\\ AutoAttack\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}PGD-\\ Latent\end{tabular}} & \begin{tabular}[c]{@{}c@{}}AdvPC-\\ Latent\end{tabular} \\ \hline
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}72.3}                                                                                                                                                                                                                                                                     & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}72.3}                                                                                                                                                                                                                                                & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}47.9}                                                                                                                                                                                                                                                                     & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}47.9}                                                                                                                                                                                                                                                \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FFF2CC}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}63.4}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}64.9}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}57.4}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}64.5}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}67.9}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}74.4}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}92.0}                          & \cellcolor[HTML]{FFF2CC}93.1                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}25.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}28.6}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}34.2}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}26.3}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}31.2}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}50.6}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}60.9}                          & \cellcolor[HTML]{FFF2CC}47.7                            \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{\multirow{-3}{*}{Pt. DP}}                                                        & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}64.6}                                                                                                                                                                                                                                                                     & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}79.9}                                                                                                                                                                                                                                                & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}32.4}                                                                                                                                                                                                                                                                     & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}47.7}                                                                                                                                                                                                                                                \\ \cline{2-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{81.3}}                                                                                                                                                                                                                                                            & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{80.4}}                                                                                                                                                                                                                                       & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{50.2}}                                                                                                                                                                                                                                                            & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{59.4}}                                                                                                                                                                                                                                       \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FFF2CC}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}\textbf{76.5}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}\textbf{68.2}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}\textbf{85.8}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}\textbf{84.0}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}\textbf{79.1}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}73.6}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}\textbf{92.9}}                 & \cellcolor[HTML]{FFF2CC}\textbf{94.3}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}\textbf{36.8}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}\textbf{50.5}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}\textbf{48.8}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}\textbf{37.5}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}\textbf{43.8}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}\textbf{59.7}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF2CC}\textbf{66.7}}                 & \cellcolor[HTML]{FFF2CC}\textbf{58.8}                   \\ \cline{3-19} 
\multicolumn{1}{|c|}{\multirow{-6}{*}{\textbf{CurveNet}}}   & \multicolumn{1}{l|}{\multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}Pt. DP\\ +S.T. (Ours)\end{tabular}}} & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{79.1}}                                                                                                                                                                                                                                                            & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{84.1}}                                                                                                                                                                                                                                       & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{44.8}}                                                                                                                                                                                                                                                            & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{57.7}}                                                                                                                                                                                                                                       \\ \hline
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}70.3}                                                                                                                                                                                                                                                                     & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}70.3}                                                                                                                                                                                                                                                & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}42.8}                                                                                                                                                                                                                                                                     & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}42.8}                                                                                                                                                                                                                                                \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FFF2CC}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}64.7}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}59.6}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}39.9}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}43.8}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}68.1}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}69.7}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}87.0}                          & \cellcolor[HTML]{FEF2CD}90.8                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}21.1}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}27.6}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}30.0}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}30.4}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}29.5}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}49.6}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}56.9}                          & \cellcolor[HTML]{FEF2CD}51.0                            \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{\multirow{-3}{*}{Pt. DP}}                                                        & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}55.7}                                                                                                                                                                                                                                                                     & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}77.2}                                                                                                                                                                                                                                                & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}30.4}                                                                                                                                                                                                                                                                     & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}46.0}                                                                                                                                                                                                                                                \\ \cline{2-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{75.8}}                                                                                                                                                                                                                                                            & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{76.0}}                                                                                                                                                                                                                                       & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{59.2}}                                                                                                                                                                                                                                                            & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{61.1}}                                                                                                                                                                                                                                       \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FFF2CC}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{77.5}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{69.4}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{80.5}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{81.0}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{77.7}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{75.5}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{92.3}}                 & \cellcolor[HTML]{FEF2CD}\textbf{94.1}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{40.1}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{51.7}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{53.1}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{41.7}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{46.0}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{64.4}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{71.9}}                 & \cellcolor[HTML]{FEF2CD}\textbf{55.9}                   \\ \cline{3-19} 
\multicolumn{1}{|c|}{\multirow{-6}{*}{\textbf{PointNet\texttt{++}~}}} & \multicolumn{1}{l|}{\multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}Pt. DP\\ +S.T. (Ours)\end{tabular}}} & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{76.8}}                                                                                                                                                                                                                                                            & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{83.1}}                                                                                                                                                                                                                                       & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{49.2}}                                                                                                                                                                                                                                                            & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{59.9}}                                                                                                                                                                                                                                       \\ \hline
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}74.0}                                                                                                                                                                                                                                                                     & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}74.0}                                                                                                                                                                                                                                                & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}57.2}                                                                                                                                                                                                                                                                     & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}57.2}                                                                                                                                                                                                                                                \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FFF2CC}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}62.8}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}69.5}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}69.6}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}62.8}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}63.1}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{74.8}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}92.4}                          & \cellcolor[HTML]{FEF2CD}\textbf{95.1}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}13.8}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}35.9}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}24.5}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}13.8}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}21.7}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}44.4}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}32.0}                          & \cellcolor[HTML]{FEF2CD}52.6                            \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{\multirow{-3}{*}{Pt. DP}}                                                        & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}67.7}                                                                                                                                                                                                                                                                     & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}79.9}                                                                                                                                                                                                                                                & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}29.1}                                                                                                                                                                                                                                                                     & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}41.6}                                                                                                                                                                                                                                                \\ \cline{2-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FBDAD7}Clean Acc & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{77.8}}                                                                                                                                                                                                                                                            & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{78.6}}                                                                                                                                                                                                                                       & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{69.6}}                                                                                                                                                                                                                                                            & \multicolumn{4}{c|}{\cellcolor[HTML]{FBDAD7}\textbf{68.2}}                                                                                                                                                                                                                                       \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{l|}{}                                                                                & \cellcolor[HTML]{FFF2CC}Adv Acc   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{67.3}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{71.4}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{87.8}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{80.9}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{70.4}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}74.7}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{92.5}}                 & \cellcolor[HTML]{FEF2CD}92.9                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{41.7}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{47.1}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{55.2}}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{31.4}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{44.4}}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{61.8}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2CD}\textbf{67.1}}                 & \cellcolor[HTML]{FEF2CD}\textbf{53.0}                   \\ \cline{3-19} 
\multicolumn{1}{|c|}{\multirow{-6}{*}{\textbf{PCT}}}        & \multicolumn{1}{l|}{\multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}Pt. DP\\ +S.T. (Ours)\end{tabular}}} & \cellcolor[HTML]{D9E7FD}Mixed Acc & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{77.1}}                                                                                                                                                                                                                                                            & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{81.8}}                                                                                                                                                                                                                                       & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{49.0}}                                                                                                                                                                                                                                                            & \multicolumn{4}{c|}{\cellcolor[HTML]{D9E7FD}\textbf{58.9}}                                                                                                                                                                                                                                       \\ \hline
\end{tabular}
    }
    \vspace{-0.5cm}
  \label{tab:adaptive_mixed}%
\end{table}



% Table generated by Excel2LaTeX from sheet 'blackbox'
\begin{table}[htbp]
  \centering
  % \vspace{-0.5cm}
  \caption{Adversarial robustness of black-box attacks on ModelNet40 under $\ell_\infty$ constraint.}
      \resizebox{0.75\linewidth}{!}{
   \begin{tabular}{|l|cc|cc|cc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{}} & \multicolumn{2}{c|}{CurveNet}                      & \multicolumn{2}{c|}{PointNet\texttt{++}~}                    & \multicolumn{2}{c|}{PCT}                           \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                  & \multicolumn{1}{c|}{Pt. DP} & Pt. Dp + S.T. (Ours) & \multicolumn{1}{c|}{Pt. DP} & Pt. Dp + S.T. (Ours) & \multicolumn{1}{c|}{Pt. DP} & Pt. Dp + S.T. (Ours) \\ \hline
SPSA                                    & \multicolumn{1}{c|}{66.6}   & \textbf{74.4}        & \multicolumn{1}{c|}{68.7}   & \textbf{73.2}        & \multicolumn{1}{c|}{69.9}   & \textbf{75.6}        \\ \hline
Nattack                                 & \multicolumn{1}{c|}{74.3}   & \textbf{78.0}        & \multicolumn{1}{c|}{76.1}   & \textbf{77.5}        & \multicolumn{1}{c|}{73.6}   & \textbf{79.7}        \\ \hline
\end{tabular}
    }
  \label{tab:blackbox}%
  % \vspace{-0.5cm}
\end{table}%


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\vspace{-0.3cm}
  \caption{Ablation study on ModelNet40 dataset with PCT and PointNet\texttt{++} backbones.}
            \setlength\tabcolsep{2pt} % default value: 6pt
        \resizebox{0.99\linewidth}{!}{
\begin{tabular}{|ccc|cccccc|cccccc|}
\hline
\multicolumn{3}{|l|}{\multirow{2}{*}{}}                                                                                                                                                                                                            & \multicolumn{6}{c|}{PCT}                                                                                                                                                                                                                                                                                                                                                                                                                                 & \multicolumn{6}{c|}{PointNet\texttt{++}~}                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \cline{4-15} 
\multicolumn{3}{|l|}{}                                                                                                                                                                                                                             & \multicolumn{3}{c|}{White-box Attack}                                                                                                                                                                                                 & \multicolumn{3}{c|}{Adaptive Attack}                                                                                                                                                                             & \multicolumn{3}{c|}{White-box Attack}                                                                                                                                                                                                 & \multicolumn{3}{c|}{Adaptive Attack}                                                                                                                                                                             \\ \hline
\multicolumn{1}{|c|}{Self-Training}                                                & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Feature \\ Distribution \\ Alignment\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Point\\ Diffusion\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Clean\\ Acc.\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Avg.\\ Adv. Acc.\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Mixed\\ Acc.\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Clean\\ Acc.\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Avg.\\ Adv. Acc.\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Mixed\\ Acc.\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Clean\\ Acc.\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Avg.\\ Adv. Acc.\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Mixed\\ Acc.\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Clean\\ Acc.\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Avg.\\ Adv. Acc.\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Mixed\\ Acc.\end{tabular} \\ \hline
\multicolumn{1}{|c|}{-}                                                            & \multicolumn{1}{c|}{-}                                                                            & -                                                         & \multicolumn{1}{c|}{\textbf{89.3}}                                        & \multicolumn{1}{c|}{30.6}                                                     & \multicolumn{1}{c|}{42.4}                                                 & \multicolumn{1}{c|}{89.3}                                                 & \multicolumn{1}{c|}{53.3}                                                     & 60.5                                                 & \multicolumn{1}{c|}{89.3}                                                 & \multicolumn{1}{c|}{30.5}                                                     & \multicolumn{1}{c|}{42.3}                                                 & \multicolumn{1}{c|}{89.3}                                                 & \multicolumn{1}{c|}{41.3}                                                     & 51.0                                                 \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Fixed\\ Threshold\end{tabular}}    & \multicolumn{1}{c|}{-}                                                                            & -                                                         & \multicolumn{1}{c|}{88.9}                                                 & \multicolumn{1}{c|}{30.7}                                                     & \multicolumn{1}{c|}{42.4}                                                 & \multicolumn{1}{c|}{87.9}                                                 & \multicolumn{1}{c|}{56.1}                                                     & 62.5                                                 & \multicolumn{1}{c|}{88.9}                                                 & \multicolumn{1}{c|}{33.6}                                                     & \multicolumn{1}{c|}{44.7}                                                 & \multicolumn{1}{c|}{\textbf{90.5}}                                        & \multicolumn{1}{c|}{59.8}                                                     & 66.0                                                 \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Adaptive\\ Threshold\end{tabular}} & \multicolumn{1}{c|}{-}                                                                            & -                                                         & \multicolumn{1}{c|}{87.9}                                                 & \multicolumn{1}{c|}{33.8}                                                     & \multicolumn{1}{c|}{44.6}                                                 & \multicolumn{1}{c|}{85.3}                                                 & \multicolumn{1}{c|}{59.8}                                                     & 64.9                                                 & \multicolumn{1}{c|}{89.1}                                                 & \multicolumn{1}{c|}{34.3}                                                     & \multicolumn{1}{c|}{45.3}                                                 & \multicolumn{1}{c|}{89.7}                                                 & \multicolumn{1}{c|}{63.4}                                                     & 68.7                                                 \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Adaptive\\ Threshold\end{tabular}} & \multicolumn{1}{c|}{$\checkmark$}                                                                            & -                                                         & \multicolumn{1}{c|}{86.6}                                                 & \multicolumn{1}{c|}{47.6}                                                     & \multicolumn{1}{c|}{55.5}                                                 & \multicolumn{1}{c|}{\textbf{89.7}}                                        & \multicolumn{1}{c|}{68.5}                                                     & 72.8                                                 & \multicolumn{1}{c|}{\textbf{89.3}}                                        & \multicolumn{1}{c|}{40.7}                                                     & \multicolumn{1}{c|}{50.5}                                                 & \multicolumn{1}{c|}{89.3}                                                 & \multicolumn{1}{c|}{69.8}                                                     & 73.7                                                 \\ \hline
\multicolumn{1}{|c|}{-}                                                            & \multicolumn{1}{c|}{-}                                                                            & PointDP                                                         & \multicolumn{1}{c|}{73.9}                                                 & \multicolumn{1}{c|}{74.7}                                                     & \multicolumn{1}{c|}{74.5}                                                 & \multicolumn{1}{c|}{74.0}                                                 & \multicolumn{1}{c|}{66.2}                                                     & 67.7                                                 & \multicolumn{1}{c|}{70.3}                                                 & \multicolumn{1}{c|}{71.2}                                                     & \multicolumn{1}{c|}{71.0}                                                 & \multicolumn{1}{c|}{70.3}                                                 & \multicolumn{1}{c|}{52.0}                                                     & 55.7                                                 \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Adaptive\\ Threshold\end{tabular}} & \multicolumn{1}{c|}{$\checkmark$}                                                                            & PointDP                                                         & \multicolumn{1}{c|}{77.6}                                                 & \multicolumn{1}{c|}{\textbf{80.1}}                                            & \multicolumn{1}{c|}{\textbf{79.6}}                                        & \multicolumn{1}{c|}{77.8}                                                 & \multicolumn{1}{c|}{\textbf{76.9}}                                            & \textbf{77.1}                                        & \multicolumn{1}{c|}{75.0}                                                 & \multicolumn{1}{c|}{\textbf{82.9}}                                            & \multicolumn{1}{c|}{\textbf{81.3}}                                        & \multicolumn{1}{c|}{75.8}                                                 & \multicolumn{1}{c|}{\textbf{77.1}}                                            & \textbf{76.8}                                        \\ \hline
\end{tabular}
}
\label{tab:ablation}%
\vspace{-0.5cm}
\end{table}

==> table/black_box.tex <==
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcc|cc|cc}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{}} & \multicolumn{2}{c|}{CurveNet} & \multicolumn{2}{c|}{PointNet++} & \multicolumn{2}{c}{PCT} \\ \cline{2-7} 
\multicolumn{1}{c}{} & PointDP & PointDP+PST(Ours) & PointDP & PointDP+PST(Ours) & PointDP & PointDP+PST(Ours) \\ \hline
SPSA & 66.6 & \textbf{74.4} & 68.7 & \textbf{73.2} & 69.9 & \textbf{75.6} \\ \hline
Nattack & 74.3 & \textbf{78.0} & 76.1 & \textbf{77.5} & 73.6 & \textbf{79.7} \\ \hline
\end{tabular}

==> table/tab_whitebox_mdlnet40.tex <==

    \begin{tabular}{cllcccccccc}
    \toprule
          &       &       & \multicolumn{4}{c|}{L\_inf}   & \multicolumn{4}{c}{L2} \\
\cmidrule{4-11}          &       &       & C\&W  & PGD   & AdvPC & \multicolumn{1}{c|}{SI\_Adv} & C\&W  & PGD   & AdvPC & KNN \\
    \midrule
    \multirow{12}[8]{*}{\begin{sideways}CurveNet\end{sideways}} & \multirow{3}[2]{*}{PointDP~\cite{sun2023critical}} & Clean Acc & 80.4  & 80.4  & 80.4  & \multicolumn{1}{c|}{80.4} & 80.4  & 80.4  & 80.4  & 80.4 \\
          &       & Adv Acc & 77.6  & 69.9  & 63.2  & \multicolumn{1}{c|}{77.2} & 75.1  & 57.9  & 62.8  & 79.2 \\
          &       & Mixed Acc & 79.0  & 75.2  & 71.8  & \multicolumn{1}{c|}{78.8} & 77.8  & 69.2  & 71.6  & 79.8 \\
\cmidrule{2-11}          & \multirow{3}[2]{*}{PointDP+PST~(Ours)} & Clean Acc & \textbf{84.5} & \textbf{84.1} & \textbf{83.6} & \multicolumn{1}{c|}{\textbf{84.0}} & \textbf{84.8} & \textbf{83.8} & \textbf{83.7} & \textbf{85.1} \\
          &       & Adv Acc & \textbf{82.3} & \textbf{77.4} & \textbf{75.3} & \multicolumn{1}{c|}{\textbf{82.6}} & \textbf{82.7} & \textbf{72.7} & \textbf{74.8} & \textbf{84.3} \\
          &       & Mixed Acc & \textbf{83.4} & \textbf{80.7} & \textbf{79.5} & \multicolumn{1}{c|}{\textbf{83.3}} & \textbf{83.8} & \textbf{78.3} & \textbf{79.3} & \textbf{84.7} \\
\cmidrule{2-11}          & \multirow{3}[2]{*}{IF-Def~\cite{wu2021ifdefense}} & Clean Acc & 78.4  & 78.9  & 80.1  & \multicolumn{1}{c|}{78.4} & 79.1  & 78.4  & 78.2  & 78.4 \\
          &       & Adv Acc & 83.1  & 54.6  & 54.2  & \multicolumn{1}{c|}{82.2} & 82.3  & 69.6  & 53.9  & 84.8 \\
          &       & Mixed Acc & 80.7  & 66.8  & 67.1  & \multicolumn{1}{c|}{80.3} & 80.7  & 74.0  & 66.1  & 81.7 \\
\cmidrule{2-11}          & \multirow{3}[2]{*}{IF-Def+PST~(Ours)} & Clean Acc & \textbf{82.5} & \textbf{80.5} & \textbf{80.7} & \multicolumn{1}{c|}{\textbf{81.2}} & \textbf{80.6} & \textbf{79.8} & \textbf{79.8} & \textbf{81.7} \\
          &       & Adv Acc & \textbf{84.3} & \textbf{67.7} & \textbf{67.6} & \multicolumn{1}{c|}{\textbf{85.6}} & \textbf{84.1} & \textbf{76.5} & \textbf{67.0} & \textbf{86.7} \\
          &       & Mixed Acc & \textbf{82.5} & \textbf{74.1} & \textbf{74.2} & \multicolumn{1}{c|}{\textbf{83.4}} & \textbf{82.3} & \textbf{78.2} & \textbf{73.4} & \textbf{84.2} \\
    \hline
    \hline
    \multirow{12}[8]{*}{\begin{sideways}PointNet++\end{sideways}} & \multirow{3}[2]{*}{PointDP~\cite{sun2023critical}} & Clean Acc & 78.1  & 78.1  & 78.1  & \multicolumn{1}{c|}{78.1} & 78.1  & 78.1  & 78.1  & 78.1 \\
          &       & Adv Acc & 74.4  & 66.9  & 62.2  & \multicolumn{1}{c|}{71.6} & 67.4  & 69.7  & 62.0  & 76.9 \\
          &       & Mixed Acc & 76.2  & 72.5  & 70.2  & \multicolumn{1}{c|}{74.8} & 72.7  & 73.9  & 70.1  & 77.5 \\
\cmidrule{2-11}          & \multirow{3}[2]{*}{PointDP+PST~(Ours)} & Clean Acc & \textbf{83.6} & \textbf{83.3} & \textbf{83.4} & \multicolumn{1}{c|}{\textbf{83.5}} & \textbf{81.9} & \textbf{83.6} & \textbf{83.6} & \textbf{83.8} \\
          &       & Adv Acc & \textbf{81.3} & \textbf{79.6} & \textbf{76.0} & \multicolumn{1}{c|}{\textbf{81.7}} & \textbf{80.0} & \textbf{78.8} & \textbf{76.0} & \textbf{82.9} \\
          &       & Mixed Acc & \textbf{82.5} & \textbf{81.4} & \textbf{79.7} & \multicolumn{1}{c|}{\textbf{82.6}} & \textbf{81.0} & \textbf{81.2} & \textbf{79.8} & \textbf{83.4} \\
\cmidrule{2-11}          & \multirow{3}[2]{*}{IF-Def~\cite{wu2021ifdefense}} & Clean Acc & 79.8  & 79.2  & 79.2  & \multicolumn{1}{c|}{79.0} & 79.2  & 79.1  & 79.2  & 79.3 \\
          &       & Adv Acc & 83.4  & 73.0  & 70.3  & \multicolumn{1}{c|}{83.5} & 81.2  & 77.2  & 71.1  & 83.9 \\
          &       & Mixed Acc & 81.6  & 76.1  & 74.8  & \multicolumn{1}{c|}{81.2} & 80.2  & 78.2  & 75.2  & 81.6 \\
\cmidrule{2-11}          & \multirow{3}[2]{*}{IF-Def+PST~(Ours)} & Clean Acc & \textbf{82.4} & \textbf{81.2} & \textbf{80.4} & \multicolumn{1}{c|}{\textbf{81.4}} & \textbf{80.7} & \textbf{81.7} & \textbf{81.3} & \textbf{81.0} \\
          &       & Adv Acc & \textbf{84.8} & \textbf{77.3} & \textbf{76.5} & \multicolumn{1}{c|}{\textbf{85.9}} & \textbf{83.0} & \textbf{80.4} & \textbf{77.3} & \textbf{84.7} \\
          &       & Mixed Acc & \textbf{83.6} & \textbf{79.3} & \textbf{78.5} & \multicolumn{1}{c|}{\textbf{83.6}} & \textbf{81.9} & \textbf{81.0} & \textbf{79.3} & \textbf{82.8} \\
    \hline
    \hline
    \multirow{12}[8]{*}{\begin{sideways}PCT\end{sideways}} & \multirow{3}[2]{*}{PointDP~\cite{sun2023critical}} & Clean Acc & 81.2  & 81.2  & 81.2  & \multicolumn{1}{c|}{81.2} & 81.2  & 81.2  & 81.2  & 81.2 \\
          &       & Adv Acc & 77.5  & 70.4  & 64.5  & \multicolumn{1}{c|}{76.2} & 75.0  & 60.0  & 65.3  & 80.4 \\
          &       & Mixed Acc & 79.3  & 75.8  & 72.8  & \multicolumn{1}{c|}{78.7} & 78.1  & 70.6  & 73.2  & 80.8 \\
\cmidrule{2-11}          & \multirow{3}[2]{*}{PointDP+PST~(Ours)} & Clean Acc & \textbf{82.4} & \textbf{83.8} & \textbf{83.4} & \multicolumn{1}{c|}{\textbf{81.0}} & \textbf{83.8} & \textbf{83.3} & \textbf{83.9} & \textbf{84.6} \\
          &       & Adv Acc & \textbf{80.1} & \textbf{75.7} & \textbf{71.5} & \multicolumn{1}{c|}{\textbf{82.8}} & \textbf{80.3} & \textbf{71.0} & \textbf{72.0} & \textbf{83.0} \\
          &       & Mixed Acc & \textbf{81.2} & \textbf{79.7} & \textbf{77.5} & \multicolumn{1}{c|}{\textbf{82.0}} & \textbf{82.1} & \textbf{77.2} & \textbf{78.0} & \textbf{83.8} \\
\cmidrule{2-11}          & \multirow{3}[2]{*}{IF-Def~\cite{wu2021ifdefense}} & Clean Acc & 80.3  & 80.9  & 81.5  & \multicolumn{1}{c|}{80.9} & 80.9  & 80.5  & 81.3  & 80.4 \\
          &       & Adv Acc & 83.2  & 60.8  & 60.4  & \multicolumn{1}{c|}{84.3} & 83.3  & 70.2  & 59.7  & 86.6 \\
          &       & Mixed Acc & 81.7  & 70.9  & 71.0  & \multicolumn{1}{c|}{82.6} & 82.1  & 75.4  & 70.5  & 83.5 \\
\cmidrule{2-11}          & \multirow{3}[2]{*}{IF-Def+PST~(Ours)} & Clean Acc & \textbf{80.2} & \textbf{82.0} & \textbf{82.5} & \multicolumn{1}{c|}{\textbf{82.3}} & \textbf{82.5} & \textbf{81.6} & \textbf{81.9} & \textbf{80.4} \\
          &       & Adv Acc & \textbf{83.5} & \textbf{69.5} & \textbf{67.4} & \multicolumn{1}{c|}{\textbf{85.0}} & \textbf{84.5} & \textbf{75.1} & \textbf{69.6} & \textbf{84.7} \\
          &       & Mixed Acc & \textbf{81.9} & \textbf{75.7} & \textbf{75.0} & \textbf{83.6} & \textbf{83.6} & \textbf{78.4} & \textbf{75.8} & \textbf{82.5} \\
    \bottomrule
    \end{tabular}%



==> table/whitebox_scanobj_mix.tex <==

\begin{tabular}{cllccc|cccc}
\hline
\multicolumn{1}{l}{} &  &  & \multicolumn{3}{c|}{\( l_\infty \)} & \multicolumn{4}{c}{\( l_2 \)} \\ \cline{4-10} 
\multicolumn{1}{l}{} &  &  & C\&W & PGD & AdvPC & C\&W & PGD & AdvPC & KNN \\ \hline
\multirow{6}{*}{\begin{sideways}CurveNet\end{sideways}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & \multicolumn{3}{c|}{42.3} & \multicolumn{4}{c}{42.8} \\
 &  & Adv Acc & 34.4 & 22.8 & 27.3 & 38 & 21.3 & 50.1 & \textbf{36.8} \\
 &  & Mixed Acc & \multicolumn{3}{c|}{31.6} & \multicolumn{4}{c}{37.8} \\ \cline{2-10} 
 & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \multicolumn{3}{c|}{\textbf{58.7}} & \multicolumn{4}{c}{\textbf{61.6}} \\
 &  & Adv Acc & \textbf{54} & \textbf{45.7} & \textbf{41} & \textbf{54.5} & \textbf{47.9} & \textbf{56.1} & \textbf{50.9} \\
 &  & Mixed Acc & \multicolumn{3}{c|}{\textbf{49.7}} & \multicolumn{4}{c}{\textbf{54.2}} \\ \hline\hline
\multirow{6}{*}{\begin{sideways}PointNet++\end{sideways}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & \multicolumn{3}{c|}{42.4} & \multicolumn{4}{c}{57.2} \\
 &  & Adv Acc & 40.6 & 18.4 & 18.8 & 27.6 & 21.6 & 53.1 & 44.2 \\
 &  & Mixed Acc & \multicolumn{3}{c|}{29.8} & \multicolumn{4}{c}{40.7} \\ \cline{2-10} 
 & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \multicolumn{3}{c|}{\textbf{54.4}} & \multicolumn{4}{c}{\textbf{62.9}} \\
 &  & Adv Acc & \textbf{51.1} & \textbf{48} & \textbf{44.5} & \textbf{45.3} & \textbf{47.2} & \textbf{53.7} & \textbf{64.9} \\
 &  & Mixed Acc & \multicolumn{3}{c|}{\textbf{49.4}} & \multicolumn{4}{c}{\textbf{54.8}} \\ \hline\hline
\multirow{6}{*}{\begin{sideways}PCT\end{sideways}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & \multicolumn{3}{c|}{49} & \multicolumn{4}{c}{47.9} \\
 &  & Adv Acc & 52.3 & 15.6 & 12.2 & 38.3 & 19.9 & 47.7 & \textbf{38.8} \\
 &  & Mixed Acc & \multicolumn{3}{c|}{32.3} & \multicolumn{4}{c}{38.5} \\ \cline{2-10} 
 & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \multicolumn{3}{c|}{\textbf{52.1}} & \multicolumn{4}{c}{\textbf{56.9}} \\
 &  & Adv Acc & \textbf{71.9} & \textbf{30.3} & \textbf{23.1} & \textbf{53.8} & \textbf{39.4} & \textbf{56.9} & \textbf{54.9} \\
 &  & Mixed Acc & \multicolumn{3}{c|}{\textbf{44.3}} & \multicolumn{4}{c}{\textbf{52.4}} \\ \hline
\end{tabular}


==> table/whitebox_scanobj_single.tex <==

% \begin{tabular}{cllcrr|crrr}
% \hline
% \multicolumn{1}{l}{} &  &  & \multicolumn{3}{c|}{\( l_\infty \)} & \multicolumn{4}{c}{\( l_2 \)} \\ \cline{4-10} 
% \multicolumn{1}{l}{} &  &  & C\&W & \multicolumn{1}{c}{PGD} & \multicolumn{1}{c|}{AdvPC} & C\&W & \multicolumn{1}{c}{PGD} & \multicolumn{1}{c}{AdvPC} & \multicolumn{1}{c}{KNN} \\ \hline\hline
% \multirow{6}{*}{\begin{sideways}CurveNet\end{sideways}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & \multicolumn{3}{c|}{72.3} & \multicolumn{4}{c}{72.3} \\
%  &  & Adv Acc & \multicolumn{1}{r}{74.8} & 71.2 & 76.0 & \multicolumn{1}{r}{74.0} & 54.3 & 76.0 & \textbf{76.1} \\
%  &  & Mixed Acc & \multicolumn{3}{c|}{73.2} & \multicolumn{4}{c}{70.5} \\ \cline{2-10} 
%  & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \multicolumn{3}{c|}{\textbf{78.2}} & \multicolumn{4}{c}{\textbf{80.4}} \\
%  &  & Adv Acc & \multicolumn{1}{r}{\textbf{84.4}} & \textbf{82.4} & \textbf{89.5} & \multicolumn{1}{r}{\textbf{79.3}} & \textbf{77.5} & \textbf{89.5} & 75.9 \\
%  &  & Mixed Acc & \multicolumn{3}{c|}{\textbf{81.6}} & \multicolumn{4}{c}{\textbf{80.5}} \\ \hline\hline
% \multirow{6}{*}{\begin{sideways}PointNet++\end{sideways}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & \multicolumn{3}{c|}{70.3} & \multicolumn{4}{c}{70.3} \\
%  &  & Adv Acc & \multicolumn{1}{r}{72.2} & 70.9 & 74.0 & \multicolumn{1}{r}{65.9} & 68.9 & 74.0 & 69.3 \\
%  &  & Mixed Acc & \multicolumn{3}{c|}{71.0} & \multicolumn{4}{c}{69.7} \\ \cline{2-10} 
%  & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \multicolumn{3}{c|}{\textbf{75.0}} & \multicolumn{4}{c}{\textbf{75.8}} \\
%  &  & Adv Acc & \multicolumn{1}{r}{\textbf{80.7}} & \textbf{85.4} & \textbf{91.5} & \multicolumn{1}{r}{\textbf{78.7}} & \textbf{81.5} & \textbf{91.3} & \textbf{75.7} \\
%  &  & Mixed Acc & \multicolumn{3}{c|}{\textbf{81.3}} & \multicolumn{4}{c}{\textbf{80.6}} \\ \hline
% \multirow{6}{*}{{\begin{sideways}PCT\end{sideways}}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & \multicolumn{3}{c|}{73.9} & \multicolumn{4}{c}{73.9} \\
%  &  & Adv Acc & \multicolumn{1}{r}{71.4} & 72.2 & 81.1 & \multicolumn{1}{r}{70.5} & 58.0 & 81.1 & \textbf{78.1} \\
%  &  & Mixed Acc & \multicolumn{3}{c|}{74.5} & \multicolumn{4}{c}{72.3} \\ \cline{2-10} 
%  & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \multicolumn{3}{c|}{\textbf{77.6}} & \multicolumn{4}{c}{\textbf{77.6}} \\
%  &  & Adv Acc & \multicolumn{1}{r}{\textbf{76.7}} & \textbf{78.7} & \textbf{89.1} & \multicolumn{1}{r}{\textbf{78.7}} & \textbf{78.7} & \textbf{84.8} & 75.9 \\
%  &  & Mixed Acc & \multicolumn{3}{c|}{\textbf{79.6}} & \multicolumn{4}{c}{\textbf{79.1}} \\ \hline
% \end{tabular}



% \begin{tabular}{cllccc|cccc}
% \hline
% \multicolumn{1}{l}{} &  &  & \multicolumn{3}{c|}{\( l_\infty \)} & \multicolumn{4}{c}{\( l_2 \)} \\ \cline{4-10} 
% \multicolumn{1}{l}{} &  &  & C\&W & PGD & AdvPC & C\&W & PGD & AdvPC & KNN \\ \hline
% \multirow{6}{*}{\begin{sideways}CurveNet\end{sideways}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & \multicolumn{3}{c|}{45} & \multicolumn{4}{c}{45} \\
%  &  & Adv Acc & 34.9 & 23.7 & 21.5 & 33.2 & 24.1 & 46.8 & \textbf{45.8} \\
%  &  & Mixed Acc & \multicolumn{3}{c|}{40} & \multicolumn{4}{c}{39.1} \\ \cline{2-10} 
%  & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \multicolumn{3}{c|}{\textbf{57.7}} & \multicolumn{4}{c}{\textbf{58.7}} \\
%  &  & Adv Acc & \textbf{54.4} & \textbf{44.3} & \textbf{41.5} & \textbf{53.1} & \textbf{44} & \textbf{59.8} & \textbf{60} \\
%  &  & Mixed Acc & \multicolumn{3}{c|}{\textbf{56.1}} & \multicolumn{4}{c}{\textbf{55.9}} \\ \hline \hline
% \multirow{6}{*}{\begin{sideways}PointNet++\end{sideways}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & \multicolumn{3}{c|}{47.4} & \multicolumn{4}{c}{47.4} \\
%  &  & Adv Acc & 37.4 & 21.4 & 16.8 & 27.7 & 31.9 & 47 & 47 \\
%  &  & Mixed Acc & \multicolumn{3}{c|}{42} & \multicolumn{4}{c}{27.6} \\ \cline{2-10} 
%  & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \multicolumn{3}{c|}{\textbf{54.7}} & \multicolumn{4}{c}{\textbf{56.9}} \\
%  &  & Adv Acc & \textbf{48.8} & \textbf{47} & \textbf{41.7} & \textbf{48.8} & \textbf{49.5} & \textbf{58.1} & \textbf{57.6} \\
%  &  & Mixed Acc & \multicolumn{3}{c|}{\textbf{51.7}} & \multicolumn{4}{c}{\textbf{52.9}} \\ \hline \hline
% \multirow{6}{*}{\begin{sideways}PCT\end{sideways}} & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & \multicolumn{3}{c|}{47.5} & \multicolumn{4}{c}{47.5} \\
%  &  & Adv Acc & 39.3 & 24.8 & 22.9 & 35.5 & 23.1 & 49.7 & \textbf{47} \\
%  &  & Mixed Acc & \multicolumn{3}{c|}{43.7} & \multicolumn{4}{c}{41.5} \\ \cline{2-10} 
%  & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \multicolumn{3}{c|}{\textbf{54.3}} & \multicolumn{4}{c}{\textbf{54.7}} \\
%  &  & Adv Acc & \textbf{48} & \textbf{40.8} & \textbf{39.8} & \textbf{50.6} & \textbf{38.6} & \textbf{58.4} & \textbf{56.9} \\
%  &  & Mixed Acc & \multicolumn{3}{c|}{\textbf{51.2}} & \multicolumn{4}{c}{\textbf{52.7}} \\ \hline
% \end{tabular}



\begin{tabular}{cllccc|cccc}
\hline
\multicolumn{1}{l}{} &  &  & \multicolumn{3}{c|}{\( l_\infty \)} & \multicolumn{4}{c}{\( l_2 \)} \\ \cline{4-10} 
\multicolumn{1}{l}{} &  &  & C\&W & PGD & AdvPC & C\&W & PGD & AdvPC & KNN \\ \hline
\multirow{6}{*}{\begin{sideways}CurveNet\end{sideways}}  & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & 45.0 & 45.0 & 45.0 & 45.0 & 45.0 & 45.0 & 45.0 \\
 &  & Adv Acc & 34.9 & 23.7 & 21.5 & 33.2 & 24.1 & 46.8 & 45.8 \\
 &  & Mixed Acc & 40.0 & 34.9 & 33.3 & 39.1 & 34.6 & 45.9 & 45.4 \\ \cline{2-10} 
 & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \textbf{57.7} & \textbf{58.3} & \textbf{58.0} & \textbf{58.7} & \textbf{58.5} & \textbf{59.7} & \textbf{59.4} \\
 &  & Adv Acc & \textbf{54.4} & \textbf{44.3} & \textbf{41.5} & \textbf{53.1} & \textbf{44.0} & \textbf{59.8} & \textbf{60.0} \\
 &  & Mixed Acc & \textbf{56.1} & \textbf{51.3} & \textbf{49.8} & \textbf{55.9} & \textbf{51.3} & \textbf{59.8} & \textbf{59.7} \\ \hline \hline
\multirow{6}{*}{\begin{sideways}PointNet++\end{sideways}}  & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & 47.4 & 47.4 & 47.4 & 47.4 & 47.4 & 47.4 & 47.4 \\
 &  & Adv Acc & 37.4 & 21.4 & 16.8 & 27.7 & 31.9 & 47.0 & 47.0 \\
 &  & Mixed Acc & 42.0 & 34.4 & 32.1 & 27.6 & 39.4 & 47.2 & 47.2 \\ \cline{2-10} 
 & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \textbf{54.7} & \textbf{57.4} & \textbf{54.9} & \textbf{56.9} & \textbf{56.2} & \textbf{57.5} & \textbf{57.1} \\
 &  & Adv Acc & \textbf{48.8} & \textbf{47.0} & \textbf{41.7} & \textbf{48.8} & \textbf{49.5} & \textbf{58.1} & \textbf{57.6} \\
 &  & Mixed Acc & \textbf{51.7} & \textbf{52.2} & \textbf{48.3} & \textbf{52.9} & \textbf{52.9} & \textbf{57.8} & \textbf{57.4} \\ \hline \hline
\multirow{6}{*}{\begin{sideways}PCT\end{sideways}}  & \multirow{3}{*}{PointDP~\cite{sun2023critical}} & Clean Acc & 47.5 & 47.5 & 47.5 & 47.5 & 47.5 & 47.5 & 47.5 \\
 &  & Adv Acc & 39.3 & 24.8 & 22.9 & 35.5 & 23.1 & 49.7 & \textbf{47.0} \\
 &  & Mixed Acc & 43.7 & 36.2 & 35.2 & 41.5 & 35.3 & 48.6 & 47.3 \\ \cline{2-10} 
 & \multirow{3}{*}{PointDP+PST(Ours)} & Clean Acc & \textbf{54.3} & \textbf{53.4} & \textbf{54.5} & \textbf{54.7} & \textbf{54.3} & \textbf{56.0} & \textbf{56.3} \\
 &  & Adv Acc & \textbf{48.0} & \textbf{40.8} & \textbf{39.8} & \textbf{50.6} & \textbf{38.6} & \textbf{58.4} & \textbf{56.9} \\
 &  & Mixed Acc & \textbf{51.2} & \textbf{47.1} & \textbf{47.2} & \textbf{52.7} & \textbf{46.5} & \textbf{57.2} & \textbf{56.6} \\ \hline
\end{tabular}

